Beyond A/B Testing: Sequential Randomization for Developing Interventions in Scaled Digital Learning Environments

Randomized experiments ensure robust causal inference that are critical to effective learning analytics research and practice. However, traditional randomized experiments, like A/B tests, are limiting in large scale digital learning environments. While traditional experiments can accurately compare two treatment options, they are less able to inform how to adapt interventions to continually meet learners' diverse needs. In this work, we introduce a trial design for developing adaptive interventions in scaled digital learning environments -- the sequential randomized trial (SRT). With the goal of improving learner experience and developing interventions that benefit all learners at all times, SRTs inform how to sequence, time, and personalize interventions. In this paper, we provide an overview of SRTs, and we illustrate the advantages they hold compared to traditional experiments. We describe a novel SRT run in a large scale data science MOOC. The trial results contextualize how learner engagement can be addressed through inclusive culturally targeted reminder emails. We also provide practical advice for researchers who aim to run their own SRTs to develop adaptive interventions in scaled digital learning environments.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> arxiv version 2/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
		Deleted indent for subsubsection (suggested by Ross Moore)
		Suppressed some obscurious warning in BibTeX processing
		Suppressed hyperrerf warnings (Paolo G. Giarrusso)
		New code for sections to help with accessibility patches
		(Ross Moore)
		Submission id, if present, is printed in anon mode
		Bug fixes

Version 1.55    Bug fixes


==> arxiv version 2/nonsense-body-from-before.tex <==
% after this it's all poo
Sequential randomization refers to the randomization of an individual multiple times throughout the course of the trial. Suppose there are two types of interventions, intervention A and intervention B. The simplest example of a sequentially randomized experiment would be: During week 1, users have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B.  During week 2 users are re-randomized to another treatment. They again have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B, independent of what happened in week 1. Hence, about 25\% of users will have received each sequence (A, A), (A,B), (B,A), (B,B), where the parenthetical notation means (week 1 treatment, week 2 treatment).

This simple sequential randomization scheme can be modified for practical and scientific reasons. Common modifications include using different time durations (e.g., re-randomize every month), increasing the number of time points (e.g., each person is randomized 10 times instead of twice), changing the number of treatments (e.g., A vs B vs C instead of A vs B, or A vs B in week 1 and C vs D in week 2), altering the randomization scheme (e.g., not having 50/50 randomization probabilities each week, or, in week 2, only re-randomizing inactive users).

Sequential randomization schemes have become relatively common in clinical settings [cites] and are becoming more prevalent in education settings [cites].  Two of the most common types of sequential randomization schemes are Sequential Multiple Assignment Randomized Trials (SMARTs) [cite Susan?s paper], and Micro-randomized Trials (MRTs) [cite Pedja?s paper]. SMART designs typically involve two randomizations, and often, the second randomization is different for different users. For example, users who didn?t respond to treatment after randomization 1 may be re-randomized, while users who did respond to treatment after randomization 1 are not re-randomized and continue with the efficacious initial treatment [cite SMART with this design]. MRTs have been mostly used in the mobile health space, where interventions (such as delivering reminders on your phone) can be delivered quickly and frequently. Because of the high frequency of interventions, MRTs are unique because they usually involve hundreds or thousand of re-randomizations.

\subsection{Comparisons to other trial designs}

Sequentially randomized trials are distinctive from many other types of common trial designs. In a typical A/B test (often called a 2-arm randomized control trial in healthcare and education), subjects are randomized one time to either intervention A or intervention B, and receive that same treatment for the entire length of the study.
http://ceur-ws.org/Vol-1688/paper-19.pdf

Sequentially randomized trials sometimes gets confused with adaptive trial designs. Adaptive trial designs are trial designs where An example of an adaptive trial design is a ?play the winner? or bandit type trial designs where, based on initial trial data collected from users, new users have different randomization probabilities which favor efficacious treatment. Another example of adaptively adjusting experimental conditions mid-trial. If intervention A starts to look much better than intervention B, then intervention B is dropped in future users? randomizations and a new intervention (B*) will be introduced.

Sequentially randomized trials are different from adaptive trial designs because in sequentially randomized trials, all users are randomized the exact same way. The randomization of new users does not change based on data collected on previous users.  Adaptive trial designs attempt to perform exploration and optimization of interventions simultaneously during the trial. Sequentially randomized trials, on the other hand, do not do any mid trial optimization. They produce a batch data set which can then be analyzed (post-trial) to understand how to optimize interventions and intervention sequences.

There are trial designs which combine sequential randomization with adaptive trial designs. Future randomizations for a particular user may change based on evidence from initial randomizations.
However, for simplicity, all of the sequentially randomized trials in this work will assume that all individuals undergo the exact same randomization scheme. 

Confirmatory trials are trials used to ensure strong evidence (or additional evidence) of a treatment?s efficacy. Confirmatory trials are typically single-randomized A/B tests where one intervention is the treatment of interest and the other intervention is the control. Confirmatory trials differ from exploratory trials. Exploratory trials are typically done in the early stages of intervention development to help researchers narrow down intervention options, understand efficacious intervention components, and learn how individuals? characteristics change intervention efficacy. Sequential randomization are useful as an exploratory trial. The goal is to explore a large number of possible treatment sequences, and learn how to personalize and optimize those sequences. After running a sequential randomized trial and designing an optimized sequence of interventions, the designed intervention sequence can be confirmed in a simple A/B confirmatory trial where the proposed intervention sequence is compared to a control.



\subsection{Applications of sequential randomization in MOOCs}

In this section I discuss a bunch of potential applications and possible interventions that could be evaluated using sequential randomization. See meeting 9/11/18 for examples.

Next, we provide a detailed example of the first-ever sequentially randomized experiment run in a MOOC, the Problem-based Email Reminder Coursera Study.


\subsection{Problem-based Email Reminder Coursera Study (PERCS)}

\subsubsection{Motivation behind PERCS}

A well-known challenge in MOOCs is low completion rates. While there are many factors contributing to MOOC dropout, the goal of PERCS was to see if dropout could be ameliorated by using weekly email reminders to motivate learners to engage with course content. These emails potentially contained a few factors intending to impact learner engagement. The email could contain a motivating data science problem to challenge the user to learn the upcoming week?s content. The email  might also contain a location specific primer and a data science problem relevant to that user?s specific culture (e.g., an Indian user might receive a problem about Bollywood or weather pattern in India). Lastly, the email may utilize growth mindset framing, a psychological framing method used to support learning.  See Table 1 for an overview of all the different kinds of emails.
 
Given all these different types of possible emails, the main research questions (ordered based on priority) were:
1. Which sequence of emails causes the highest rate of completion?
2. Which type of data science problem email (no email, no problem, generic data science problem, or culturally relevant data science problem) is most effective for bringing learners back to the course?
3. Are certain data science problem emails more or less effective for active learners?        
4.Does growth mindset framing improve an emails ability to bring learners back to the course?

\subsubsection{Design of PERCS}

A sequentially randomized factorial trial design was an effective method to jointly address the main research questions of PERCS.  At the end of weeks one, two, and three of the four-week long MOOC, learners were randomly assigned to receive one of four different email categories: an email message with a problem that reflects their geo-cultural situation based on IP address analysis (personalized problem condition), an email with a generic non-culture specific problem (global problem condition), an email with no problem (no problem condition), or no email at all (no email condition). These learners were also randomly assigned to have their email be framed with a growth mindset or without a growth mindset. The growth mindset piece crossed with the three email categories makes each week of PERCS a 2x3 factorial design with an additional control condition of no email. See table 1 for each week?s factorial design and randomization probabilities.
 
The most novel aspect of PERCS is the sequential randomization. That is, a particular learner does not get randomized to one email condition and remain in that treatment condition for all 3 weeks (as is typically done in experiments). Instead, each week, a learner is re-assigned (with the same randomization probabilities) to a different email condition. The randomizations across weeks are independent. Hence, in PERCS, there are $7^3$ possible trajectories of emails, for example, (A,A,A) (A,B,C) (A, A, G), where where the parenthetical notation means (week 1 treatment, week 2 treatment, week 3 treatment) with letters corresponding to treatment in Table 1.

\subsubsection{Participation in PERCS}

All learners who signed up for the Introduction to Applied Data Science with Python course on Coursera between the times of April 1, 2018 to June 10, 2018 participated in PERCS. A total of 15,037 unique learners were sent 28,446 emails. 

\subsubsection{AB Testing Version of PERCS}

To highlight the advantages of sequential randomization within PERCS, PERCS will be compared to the single-randomized, AB testing version of PERCS (called PERCS-AB). PERCS-AB has the exact same randomization probabilities as PERCS, however in PERCS-AB, prior to the start of week two, learners are randomized to one of the 7 email types, and are sent that exact same email type for the subsequent 3 weeks. Hence, there are only 7 possible trajectories (A, A, A), (B,B,B) ?, (G,G,G).

\section{Discovering an optimal sequence of treatments}
Is it better to space out review problems by?? 
For PERCSs, which sequence of emails (and no emails) leads to most returns to the course?
All of these questions are asking about optimizing and comparing sequences of interventions.

Sequentially randomized trials provide data that allows experimenters to compare different sequences of interventions. By re-randomizing learners, learners receive a variety of treatment sequences. In PERCS, for example, with the large sample size, there are learners who have the trajectory (A, A, A), (A, A, B), (A, B, B), (B, A, B), etc. For the $7^3$ possible sequences of treatments, there are learners randomly assigned to each of those sequences.

By having learners randomized to all of these different trajectories, researchers are now able to compare different sequences of treatment. For example, researchers could compare the effects on course activity of (No email, No problem growth mindset email, Culturally personalized non-growth mindset email) to (Global problem growth mindset email, Culturally personalized growth mindset email, No email), by simply comparing the course activity of users randomized to these 2 sequences.

Often times, researcher are not interested in such specific sequence comparisons. Instead, they are interested in questions about sequences of groups of interventions. In this case, one could perform similar comparisons, but combining users over all of these groups. For example, in PERCS, we were curious about how often reminder emails should be sent. Is it better to space emails out weekly or bi-weekly? To answer this question, we could compare course activity of users under the sequence ({B, C, D, E, F, G}, {A}, {B-G}), i.e., the trajectory which spaces emails out by 2-weeks, to (B + C + D + E + F + G, B + C + D + E + F + G, B + C + D + E + F + G), i.e., the trajectory which sends emails every week.  The sample size for this comparison will be much larger than for the single sequence comparisons.

In addition to comparing groups of sequences, researchers might only be interested in comparing sequences for a small number of time points. For example, in PERCS, we were curious if the effects of week two 2 problem-based emails on course activity were different based on what type of problem based email the user had received in week one1. Specifically, does getting no email vs no problem email vs problem based email in week one1 change the benefits of problem-based emails in week 2?  To answer this question, we compare course activity in week 2 of users receiving sequences (A, D + E + F + G, all), (B + C, D + E + F + G, all), and (D + E + F + G, D + E + F + G, all). Notice how we were not concerned with anything occurring in week three3, so we include sequences with any email in week three3.

In PERCS-AB, learners are only randomized to 7 possible trajectories (A, A, A), (B,B,B) ?, (G,G,G). Hence, comparisons can only be done between these 7 trajectories. If there was any benefit to receiving different interventions, in a different order, this could not be discovered by PERCS-AB. Notice also that all of the comparisons of PERCS-AB cancould be done with data collected through PERCS, though this comes at the cost of a reduced (though the sample size. This tradeoff demonstrations again why sequential random trials are especially well situated for MOOC experimentation will be much smaller).

\subsection{Results from PERCS}

For PERCS, we were most interested in understanding how to best sequence and space out emails with problems and emails without problems. We were not sure if users would be motivated by only problem based emails, or if, some weeks they would want no-problem based email reminders or no emails at all.  Specifically, we interested in understanding the sequential differences between the groups: 1) no emails (A), 2) no problem emails (B+C), and 3) problem emails (D+E+F+G). Each week, a user could have received one of these 3 types of emails, providing $3^3$ = 27 sequences to compare (i.e., (1,1,1), (1,1,2), (1,1,3), (1,2,1), (1,2,2), (1,2,3), ?, (3,3,2), (3,3,3)). For users in each of these sequences, we create a confidence interval for the log number of course clicks throughout the entire course. The results are in table blah

Table showing top 5 sequences and bottom 5 sequences

<Insert conclusions to be made based on table>

\section{Average treatment effects at various time points}
Instead of being interested in a sequence of interventions, researchers might want to know about the average effect of an intervention at a particular time point. To understand spaced repetition, researchers may want to know the effect of introducing review content in the 3rd week of the course? In PERCS, we wanted to know the effect of culturally personalized problem emails in weeks 2 on the subsequent week?s course activity. We also wanted to know the effect of including growth mindset framing in emails in week 3.

Sequentially randomized experiments permit the estimation of average treatment effects at various time points, where the averaging is over all prior treatments received. By re-randomizing individuals, we can separately estimate average effects at each time point and break confounding from previous time points. For example, in PERCS, if we wanted to know the average effect of culturally personalized problem emails in week 3 compared to global problem emails in week 3, we compare users receiving (all, all, F + G) to users receiving (all, all, D+E). By doing this comparison, we average over all treatments delivered prior to week 3, and isolate the effect of interest to problem emails only in week 3. 

In PERCS-AB, such a comparison is impossible. We could only compare the effects of culturally personalized problem emails for all 3 weeks, to global problem emails for all 3 weeks (F+G, F+G, F+G) vs (D+E, D+E, D+E). The effect estimated in PERCS-AB is a compounding effect of culturally problem-based and global problem-based emails instead of an average effect isolated to week 3.

In sequentially randomized trials average treatment effects can also be estimated for outcomes measured after the next re-randomization (sometimes called delayed effects).  For example, for PERCS, in addition to understanding the average effect of culturally personalized problem emails in week 2, on week 3 course activity, we are also able to understand the average effect of culturally personalized problem emails in week 2, on week 4 course activity (and other outcomes such as course completion). In this estimation, one would average over both week 1 treatment and week 3 treatment. This delayed effect cannot be estimated in PERCS-AB since, with no re-randomization after week 2, the estimate will be confounded by treatment in week 3.

\subsection{The Difference Between Average Treatment Effects and Sequence Effects}

Research questions on average treatment effects often seem similar to questions regarding sequence effects. In order to elucidate the difference, below are 3 types of questions that may be of interest to researchers:

1. What is the effect on week 3 course activity of getting any email in week 2, after not receiving an email prior? Compare (A, B+C+D+E+F+G, all) vs (A, A, all)

2. What is the average effect on week 3 course activity of getting any email in week 2, on average (averaging over all prior treatment)? Compare (all, B+C+D+E+F+G, all) vs (all, A, all)

3. What is the effect on week 3 course activity, of getting emails each week? Compare (B+C+D+E+F+G, B+C+D+E+F+G, B+C+D+E+F+G) vs (A, A, A)

Questions 1 and 3 are questions of comparing sequences of treatments, while question 2 is about average treatment effects. Note that all 3 questions can be answered by PERCS, but only questions 3 can be answered by PERCS-AB.

Also, one advantage of analyzing average treatment effects is that the sample size is typically larger than comparing sequences of treatments. The number of users used to make the comparison is much larger, since the comparison doesn?t restrict users based on what they received before or after the given week of interest.

\subsection{Results from PERCS}

In PERCS, we were interested in two average treatment effects. We wanted to know the effect on the subsequent week?s course activity of culturally personalized problem emails in weeks 1, 2, and 3. We also wanted to know the effect of including growth mindset framing in emails in weeks 1, 2, 3.

PERCS, throw in tables for JLS paper
Also say growth mindset didn?t appear to have an effect. Maybe put in table here just to show comparison.

Table 3:Log odds ratios for logistic regression model with the outcome being the binary measure of (1) the user clicks anything in the course during the week after receiving an email vs (0) the user does not click anything in the course in the subsequent week. The baseline is no email. 

\section{Personalization of interventions with Sequentially Randomized Trials}

MOOCs are notable for the high degree of diversity across their learner populationsIn MOOCs, there are a large amount of diversity between learners. In addition, as learners progress through a course, there is even diversity within a learner:; a learner?s engagement patterns may evolve from the initial weeks of a course to later weeks as their goals, knowledge, and experience changea learner?s engagement in the first week of the course can change in later weeks.   Due to this diversity, interventions may not always have the same effect. If anone intervention works for a specificone user at a givenone time, that intervention may not be effective it does not mean it will work for a different user, or even the same user, at a different time.  Personalizing treatment, by discovering when and for whom certain treatments are most effective, is critical. 

In literature, learning how to personalize treatment is synonymous with discovering moderators [cite]. Moderators are subject-specific variables which change the efficacy of anthe intervention. For example, if a MOOC intervention works better for older users than younger users, then age is a moderator and can then be used to personalize the intervention; after discovering age is a moderator, one may only deliver the intervention to older learners only. Some moderators can be discovered using A/B trials, however, sequentially randomized trials permits the discovery of two other types of moderators: additional baseline sequence moderators and mid-course moderators.

\subsection{Baseline sequence moderators}

Baseline variables are variables measured prior to the first treatment randomization and which can be treated as fixed for the period of a study. Baseline variables include learner characteristics (e.g., gender, location, age, prior courses taken) and course activity measured prior to the first randomization (e.g., whether the users has taken the course previously, scores on early assignments, survey responses at the beginning of the course). Often these variables moderate the effect of treatments and can be used for personalization. Discovering baseline moderators helps understand how to personalize interventions to account for diversity between different learners.

Sequential randomized trials and A/B tests both permit the discovery of baseline moderators. However, in sequential randomized trials, because users receiving a larger variety of sequences of interventions, this permits the discovery of baseline moderators for a larger number of intervention sequences, leading to a richer and more specific understanding of the moderating effects of various learner characteristics.

As an exampleTo exemplify, in both PERCS and PERCS-AB, one could answer the question: is the effect of 3 weeks of culturally personalized problem emails (compared to 3 weeks of non-personalized problem emails) different for lndian learners compared to US learners? However, in PERCS, one is able to evaluate the moderation of learners? location on a larger variety of treatment sequence comparisons. Indeed, the PERCS design allows an experimenter to evaluate the moderation of location on every possible sequence of interventions in the space under consideration.  One could also answer: is the effect of sequences which vary personalized and non-personalized problem emails (compared to 3 weeks of non-personalized problem emails) different for lndian learners compared to US learners? PERCS-AB is not able to answer this second question since no users are re-randomized to receive both personalized and non-personalized emails throughout the course. PERCS-AB is only able to evaluate moderation of baseline variables on the small number of sequences in the trial.

\subsection{Mid-course moderators}

Baseline moderators are important for personalizing initial treatment (or treatment sequences), however, understanding how to change treatment based on variables measured throughout the course --, i.e., mid-course moderators --, is critical. Discovering mid-course moderators tells practitioners how to personalize interventions throughout the course to account for diversity both between different users and within a user over time. 

Unlike A/B tests, sequential randomized trials permit the discovery of mid-course moderators. Statistically, due to bias introduced when including post-randomization variables in analyses, one can only discover moderator variables measured prior to randomization. By re-randomizing in sequentially randomized trials, moderators measured before each of the randomizations (which now includes mid-course data) can be discovered. 
<Should I further explain here the specifics, like I still have to preserve ordering, I can only assess there moderation on future treatment>

To exemplify, in PERCS, we hypothesized that growth mindset framing in emails sent at the end of week three only works well for students who were inactive during week 3, because they would benefit from the growth mindset encouragement. Because users were randomized again at the end of week 3, we can use PERCS data to assess how week 3 activity moderates the effect of growth mindset emails (sent at the end week 3) on week 4 activity. In PERCS-AB, week three course activity cannot be assessed as a moderator in PERCS-AB since it was measured after the one and only randomization in week one. 

We can also evaluate mid-course moderators that include previous treatment. For example, we may think that responsiveness to previous treatment could inform how to personalize future treatment. Those that were responsive should continue getting the same treatment while those that were non-responsive should get assigned different treatment. In PERCS, we hypothesized that growth mindset emails are more effective for users indicating they liked growth mindset in the previous week and users indicating they did not like non-growth mindset in the previous week. More specifically, there are four groups of learners: Group 1 are learners who received growth mindset framing in week one and had course activity in week two (i.e., growth mindset responders), Group 2 are learners who received growth mindset framing in week one and had no course activity in week two (i.e., growth mindset non-responders), Group 3 are learners who received no growth mindset framing in week one and had course activity in week two (i.e., no growth mindset responders), Group 4 are learners who received no growth mindset framing in week one and had no course activity in week two (i.e., no growth mindset non-responders). We expected growth mindset framing in week two emails to benefit Groups 1 and 4 more than Groups 2 and 3. By re-randomizing at the end of week two, we assess moderation by comparing treatment effects of growth mindset framing in week two emails for Groups 1 and 4 vs Groups 2 and 3.

Discovering how to personalize based on mid-course activity is one of the major benefits of sequential randomized trials. There are many other examples: . These discoveries allow educators to adapt content and interventions to meet the needs of learners as they dynamically transition throughout the course. Also, as learning content optimization starts to happen in real-time (i.e., reinforcement learning), knowing which real-time variables to measure and use for online optimization is critical. Sequentially randomized trials permit this discovery.

sentence like this herev but for within leaners: Discovering baseline moderators helps understand how to personalize interventions to account for diversity between different learners.

\subsection{Results from PERCS}

For PERCS, we were most interested in previous week?s course activity as a mid-course moderator. We wanted to see how different types of emails effect active and inactive users differently. Problem based emails may encourage or discourage inactive users. Not sure
Figure blah shows the results
<Insert conclusions to be made based on table>

\section{implications for practice}

This section outlines some useful considerations for researchers who are interested in designing and running sequential randomized trials for scaled learning environments. First, before thinking about trial specifics, researchers should always remember that experiments are created to inform scientific and answer questions about interventions. Deciding if a sequential randomized trial is the correct trial design depends purely upon the scientific questions of interest. For example, if researchers are not interested in understanding interventions which adapt and change throughout the course, running a sequential randomized trial is unnecessary. In PERCS, for example, if we, apriori, only cared about comparing interventions which send the same email all three weeks (because we think that what email was best in week one will be the best email in weeks two and three), then PERCS-AB would be a sufficient trial design.

If running a sequential randomized trial is best, there are also important considerations for creating the design.  All intervention sequences in a sequential randomized trial should be useful, feasible, and scalable. It is useless to evaluate intervention sequences which could never be done in practice or which are knowingly deleterious. For example, suppose a researcher was curious about optimal ordering of course content and, in turn, sequentially randomized learners to various sequences of content. If content B requires information taught in content A, none of the sequences in the experiment should place content B before content A. For another example, in PERCS, because currently there is not a completely automated way to send emails at any time, we only sent emails once a week. We did not explore the possibility of send emails many times per week (e.g., re-randomizing email sending every day) because, in practice, interventions which require manual email sending every day would not be feasible for MOOC instructors.

As in any other trial design, sample size and power calculations are important for sequentially randomized trials. Sample size calculations should be based off of the most important research questions the trial intends to answer. Since there are a larger number of possible treatment sequences in a sequentially randomized trial, calculating power and sample size requires researchers to consider which subset of users will be randomized to the sequences of interest. Once understanding which users will be used in the given comparison, sample size calculations are similar to A/B test sample size formulae for both comparing interventions and discovering moderators. 
Due to there more divisions of users to various sequences and a richer set of answerable research questions, sample sizes usually need to be larger for sequentially randomized trials (compared to A/B tests). If a researcher were only really interested in comparing two sequences of interventions and had  limited sample size, then it may be best to run an A/B test on those two sequences and forgo answers to other questions. The research may also consider changing the randomization probabilities. For example, in PERCS, if we mostly cared about comparing culturally personalized problem emails to global problem emails, we might change the weekly randomization probabilities in Table 1 to favor these two interventions.



\newpage

\section{Page 1 for figures and tables}

\newpage

\section{Page 2 for figures and tables}

\newpage

\section{Page 3 for figures and tables}

\newpage

\section{Page for references}



\newpage
\newpage
\section{Introduction}

The \textit{proceedings} are the records of a conference.\footnote{This
  is a footnote}  ACM seeks
to give these conference by-products a uniform, high-quality
appearance.  To do this, ACM has some rigid requirements for the
format of the proceedings documents: there is a specified format
(balanced double columns), a specified set of fonts (Arial or
Helvetica and Times Roman) in certain specified sizes, a specified
live area, centered on the page, specified size of margins, specified
column width and gutter size.

\section{The Body of The Paper}
Typically, the body of a paper is organized into a hierarchical
structure, with numbered or unnumbered headings for sections,
subsections, sub-subsections, and even smaller sections.  The command
\texttt{{\char'134}section} that precedes this paragraph is part of
such a hierarchy.\footnote{This is a footnote.} \LaTeX\ handles the
numbering and placement of these headings for you, when you use the
appropriate heading commands around the titles of the headings.  If
you want a sub-subsection or smaller part to be unnumbered in your
output, simply append an asterisk to the command name.  Examples of
both numbered and unnumbered headings will appear throughout the
balance of this sample document.

Because the entire article is contained in the \textbf{document}
environment, you can indicate the start of a new paragraph with a
blank line in your input file; that is why this sentence forms a
separate paragraph.

\subsection{Type Changes and {\itshape Special} Characters}

We have already seen several typeface changes in this sample.  You can
indicate italicized words or phrases in your text with the command
\texttt{{\char'134}textit}; emboldening with the command
\texttt{{\char'134}textbf} and typewriter-style (for instance, for
computer code) with \texttt{{\char'134}texttt}.  But remember, you do
not have to indicate typestyle changes when such changes are part of
the \textit{structural} elements of your article; for instance, the
heading of this subsection will be in a sans serif\footnote{Another
  footnote here.  Let's make this a rather long one to see how it
  looks.} typeface, but that is handled by the document class file.
Take care with the use of\footnote{Another footnote.}  the
curly braces in typeface changes; they mark the beginning and end of
the text that is to be in the different typeface.

You can use whatever symbols, accented characters, or non-English
characters you need anywhere in your document; you can find a complete
list of what is available in the \textit{\LaTeX\ User's Guide}
\cite{Lamport:LaTeX}.

\subsection{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of
the three are discussed in the next sections.

\subsubsection{Inline (In-text) Equations}
A formula that appears in the running text is called an
inline or in-text formula.  It is produced by the
\textbf{math} environment, which can be
invoked with the usual \texttt{{\char'134}begin\,\ldots{\char'134}end}
construction or with the short form \texttt{\$\,\ldots\$}. You
can use any of the symbols and structures,
from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a
few examples of in-text equations in context. Notice how
this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsubsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols
and structures available in \LaTeX\@; this section will just
give a couple of examples of display equations in context.
First, consider the equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\subsection{Citations}
Citations to articles~\cite{bowman:reasoning,
clark:pct, braams:babel, herlihy:methodology},
conference proceedings~\cite{clark:pct} or maybe
books \cite{Lamport:LaTeX, salas:calculus} listed
in the Bibliography section of your
article will occur throughout the text of your article.
You should use BibTeX to automatically produce this bibliography;
you simply need to insert one of several citation commands with
a key of the item cited in the proper location in
the \texttt{.tex} file~\cite{Lamport:LaTeX}.
The key is a short reference you invent to uniquely
identify each work; in this sample document, the key is
the first author's surname and a
word from the title.  This identifying key is included
with each item in the \texttt{.bib} file for your article.

The details of the construction of the \texttt{.bib} file
are beyond the scope of this sample document, but more
information can be found in the \textit{Author's Guide},
and exhaustive details in the \textit{\LaTeX\ User's
Guide} by Lamport~\shortcite{Lamport:LaTeX}.

This article shows only the plainest form
of the citation command, using \texttt{{\char'134}cite}.

Some examples.  A paginated journal article \cite{Abril07}, an enumerated
journal article \cite{Cohen07}, a reference to an entire issue \cite{JCohen96},
a monograph (whole book) \cite{Kosiur01}, a monograph/whole book in a series (see 2a in spec. document)
\cite{Harel79}, a divisible-book such as an anthology or compilation \cite{Editor00}
followed by the same example, however we only output the series if the volume number is given
\cite{Editor00a} (so Editor00a's series should NOT be present since it has no vol. no.),
a chapter in a divisible book \cite{Spector90}, a chapter in a divisible book
in a series \cite{Douglass98}, a multi-volume work as book \cite{Knuth97},
an article in a proceedings (of a conference, symposium, workshop for example)
(paginated proceedings article) \cite{Andler79}, a proceedings article
with all possible elements \cite{Smith10}, an example of an enumerated
proceedings article \cite{VanGundy07},
an informally published work \cite{Harel78}, a doctoral dissertation \cite{Clarkson85},
a master's thesis: \cite{anisi03}, an online document / world wide web
resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03}
and \cite{Lee05} and (Case 3) a patent \cite{JoeScientist001},
work accepted for publication \cite{rous08}, 'YYYYb'-test for prolific author
\cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might contain
'duplicate' DOI and URLs (some SIAM articles) \cite{Kirschmer:2010:AEI:1958016.1958018}.
Boris / Barbara Beeton: multi-volume works as books
\cite{MR781536} and \cite{MR781537}.

A couple of citations with DOIs: \cite{2004:ITE:1009386.1010128,
  Kirschmer:2010:AEI:1958016.1958018}.

Online citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.


\subsection{Tables}
Because tables cannot be split across pages, the best
placement for them is typically the top of the page
nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and
the table caption.  The contents of the table itself must go
in the \textbf{tabular} environment, to
be aligned properly in rows and columns, with the desired
horizontal and vertical rules.  Again, detailed instructions
on \textbf{tabular} material
are found in the \textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed
output of this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more desirable.
Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.


\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}
% end the environment with {table*}, NOTE not {table}!

It is strongly recommended to use the package booktabs~\cite{Fear05}
and follow its main principles of typography with respect to tables:
\begin{enumerate}
\item Never, ever use vertical rules.
\item Never use double rules.
\end{enumerate}
It is also a good idea not to overuse horizontal rules.


\subsection{Figures}

Like tables, figures cannot be split across pages; the best placement
for them is typically the top or the bottom of the page nearest their
initial cite.  To ensure this proper ``floating'' placement of
figures, use the environment \textbf{figure} to enclose the figure and
its caption.

This sample document contains examples of \texttt{.eps} files to be
displayable with \LaTeX.  If you work with pdf\LaTeX, use files in the
\texttt{.pdf} format.  Note that most modern \TeX\ systems will convert
\texttt{.eps} to \texttt{.pdf} for you on the fly.  More details on
each of these are found in the \textit{Author's Guide}.

\begin{figure}
\includegraphics{fly}
\caption{A sample black and white graphic.}
\end{figure}

\begin{figure}
\includegraphics[height=1in, width=1in]{fly}
\caption{A sample black and white graphic
that has been resized with the \texttt{includegraphics} command.}
\end{figure}


As was the case with tables, you may want a figure that spans two
columns.  To do this, and still to ensure proper ``floating''
placement of tables, use the environment \textbf{figure*} to enclose
the figure and its caption.  And don't forget to end the environment
with \textbf{figure*}, not \textbf{figure}!

\begin{figure*}
\includegraphics{flies}
\caption{A sample black and white graphic
that needs to span two columns of text.}
\end{figure*}


\begin{figure}
\includegraphics[height=1in, width=1in]{rosette}
\caption{A sample black and white graphic that has
been resized with the \texttt{includegraphics} command.}
\end{figure}

\subsection{Theorem-like Constructs}

Other common constructs that may occur in your article are the forms
for logical constructs like theorems, axioms, corollaries and proofs.
ACM uses two types of these constructs:  theorem-like and
definition-like.

Here is a theorem:
\begin{theorem}
  Let $f$ be continuous on $[a,b]$.  If $G$ is
  an antiderivative for $f$ on $[a,b]$, then
  \begin{displaymath}
    \int^b_af(t)\,dt = G(b) - G(a).
  \end{displaymath}
\end{theorem}

Here is a definition:
\begin{definition}
  If $z$ is irrational, then by $e^z$ we mean the
  unique number that has
  logarithm $z$:
  \begin{displaymath}
    \log e^z = z.
  \end{displaymath}
\end{definition}

The pre-defined theorem-like constructs are \textbf{theorem},
\textbf{conjecture}, \textbf{proposition}, \textbf{lemma} and
\textbf{corollary}.  The pre-defined de\-fi\-ni\-ti\-on-like constructs are
\textbf{example} and \textbf{definition}.  You can add your own
constructs using the \textsl{amsthm} interface~\cite{Amsthm15}.  The
styles used in the \verb|\theoremstyle| command are \textbf{acmplain}
and \textbf{acmdefinition}.

Another construct is \textbf{proof}, for example,

\begin{proof}
  Suppose on the contrary there exists a real number $L$ such that
  \begin{displaymath}
    \lim_{x\rightarrow\infty} \frac{f(x)}{g(x)} = L.
  \end{displaymath}
  Then
  \begin{displaymath}
    l=\lim_{x\rightarrow c} f(x)
    = \lim_{x\rightarrow c}
    \left[ g{x} \cdot \frac{f(x)}{g(x)} \right ]
    = \lim_{x\rightarrow c} g(x) \cdot \lim_{x\rightarrow c}
    \frac{f(x)}{g(x)} = 0\cdot L = 0,
  \end{displaymath}
  which contradicts our assumption that $l\neq 0$.
\end{proof}

\section{Conclusions}
This paragraph will end the body of this sample document.
Remember that you might still have Acknowledgments or
Appendices; brief samples of these
follow.  There is still the Bibliography to deal with; and
we will make a disclaimer about that here: with the exception
of the reference to the \LaTeX\ book, the citations in
this paper are to articles which have nothing to
do with the present subject and are used as
examples only.
%\end{document}  % This is where a 'short' article might terminate



\appendix
%Appendix A
\section{Headings in Appendices}
The rules about hierarchical headings discussed above for
the body of the article are different in the appendices.
In the \textbf{appendix} environment, the command
\textbf{section} is used to
indicate the start of each Appendix, with alphabetic order
designation (i.e., the first is A, the second B, etc.) and
a title (if you include one).  So, if you need
hierarchical structure
\textit{within} an Appendix, start with \textbf{subsection} as the
highest level. Here is an outline of the body of this
document in Appendix-appropriate form:
\subsection{Introduction}
\subsection{The Body of the Paper}
\subsubsection{Type Changes and  Special Characters}
\subsubsection{Math Equations}
\paragraph{Inline (In-text) Equations}
\paragraph{Display Equations}
\subsubsection{Citations}
\subsubsection{Tables}
\subsubsection{Figures}
\subsubsection{Theorem-like Constructs}
\subsubsection*{A Caveat for the \TeX\ Expert}
\subsection{Conclusions}
\subsection{References}
Generated by bibtex from your \texttt{.bib} file.  Run latex,
then bibtex, then latex twice (to resolve references)
to create the \texttt{.bbl} file.  Insert that \texttt{.bbl}
file into the \texttt{.tex} source file and comment out
the command \texttt{{\char'134}thebibliography}.
% This next section command marks the start of
% Appendix B, and does not continue the present hierarchy
\section{More Help for the Hardy}

Of course, reading the source code is always useful.  The file
\path{acmart.pdf} contains both the user guide and the commented
code.

\begin{acks}
  The authors would like to thank Dr. Yuhua Li for providing the
  MATLAB code of the \textit{BEPS} method.

  The authors would also like to thank the anonymous referees for
  their valuable comments and helpful suggestions. The work is
  supported by the \grantsponsor{GS501100001809}{National Natural
    Science Foundation of
    China}{http://dx.doi.org/10.13039/501100001809} under Grant
  No.:~\grantnum{GS501100001809}{61273304}
  and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
    Scientists' Support Program}.

\end{acks}

==> arxiv version 2/old_main_body.tex <==
\section{Introduction}\label{sec:introduction}

In order to continually improve learner experience and maintain engagement, scaled digital learning environments (SDLEs), such as Massively Open Online Courses (MOOCs), intelligent tutoring systems, and open-ended digital educational games, utilize \textit{interventions}. Interventions are modifications made to the learning environment or learners' experience of it, including changing current course content, prompting users to return to the course, or providing additional learning resources (e.g.,\cite{Davis_2018}). It is common to find interventions which are technological, pedagogical, or programmatic in their implementation.

In SDLEs, there is typically diversity both \textit{between} learners (e.g., different learners have different needs) \cite{Kizilcec_2017}, and \textit{within} a learner over time (e.g., a learner's engagement may change throughout a course) \cite{Kizilcec_2013}. To accommodate this diversity, interventions should be adaptive. \textit{Adaptive interventions} can change based on the type of learner (to account for diversity between learners) and change as a learner progresses through the course (to account for diversity within a learner) \cite{almirall_2018}. For example, consider an intervention which introduces review problems throughout a course. The frequency of review problems might adapt based on the week (e.g., learners may not need to review as often in later weeks). The frequency of review might also adapt based on the learner's performance (e.g., building upon work on theories of \emph{spaced repetition} \cite{reynolds1964effects}).

Due to the large number of users and ease of content manipulation in SDLEs, randomized controlled trials (e.g., A/B tests) are often used to evaluate education intervention options (e.g., learning activity). Typically, these experiments are single-randomized trials where each subject is randomized once, and assigned to a single intervention option for the entire trial. However, when the goal is to design a high-quality adaptive intervention in SDLEs, researchers may have important questions about the sequencing, timing, and personalization of intervention options which cannot be answered by A/B tests.  

In this work, we discuss and demonstrate the advantages of an experimental design for developing high-quality adaptive interventions in SDLEs: the \textit{sequential randomized trial} (SRT). In SRTs, a subject is randomized several times to different intervention options throughout the experiment. Sequential randomization is beneficial over one-time randomization for several reasons.  Firstly, by re-randomizing, subjects receive a variety of intervention sequences, and these various sequences can be compared to discover the optimal intervention sequence.  Secondly, instead of only being able to assess the overall effect of getting one particular treatment, sequential randomization lets researchers discover effects at smaller time-scales (e.g., treatment A does better in week 2 of the course, but treatment B does better in week 3 of the course). These discoveries inform at what time points certain interventions are most effective. Thirdly, re-randomization permits the discovery of important variables measured throughout the course for adapting and personalizing an intervention. As opposed to only being able to discover baseline personalization variables (e.g., treatment A works better for women), we can also discover mid-course personalization variables (treatment A works better for subjects with who have been active in the course during the previous day).
 
%SRTs are particularly advantageous when aiming to develop an adaptive intervention in SDLEs. First, SRTs inform how to adapt interventions to meet the needs of all learners at all times within the diverse learner population of an SDLE. Second, the fully computer-mediated nature of many SDLEs means that there are typically a large number of possible modifications and intervention options. SRTs can maximally leverage the large sample sizes of SRTs, sometimes on the order of tens of thousands of learners \cite{Kizilcec_2017}, by comparing, with power, a larger variety of treatment sequences than an A/B test. For example, course designers can modify the ordering of course content, as well as layout, appearance (color, texture), arrangement, and default settings of interfaces. Third, SRTs are beneficial for research in SDLEs from a practical perspective. In clinical or classroom settings, reassignment of intervention options adds a layer of complexity, making intervention delivery difficult. In SDLEs, where interventions can be delivered quickly and at scale, the burden of re-randomization and delivering a variety of intervention options is minimized. SRTs leverage this lower cost of re-randomization within a trial by repeatedly re-assigning users to new treatments.  

%SRTs are particularly useful as exploratory trials (as opposed to confirmatory), to help researchers narrow down intervention options and discover the best (which can then be further validated). SDLEs are also better able to implement a personalized adaptive intervention based on results of a SRT. In face-to-face or blended learning environments it is often impractical to deliver personalized interventions to each student, as the nature of the face-to-face experience tends to preclude individual-level learning from the instructor. 

The paper is structured as follows. First, we provide an overview of related prior work on experimentation and personalized interventions in SDLEs in Section \ref{sec:prior-work}. In Section \ref{sec:seqential-randomization}, we formally introduce SRTs and compare them to other common trial designs.
 In Section \ref{sec:srt_examples}, to motivate the design we describe a novel
 %\footnote{The authors are not aware of any previous SRT designs being used in MOOC research to date.}
 SRT performed in MOOCs, the Problem-based Email Reminder Coursera Study (PERCS). 
 This was an experiment aiming to
 improve student retention in an online course by developing a high-quality adaptive email intervention which 
 leverages aspects of cultural diversity and inclusion \cite{Aceves_2014a}. This case study both serves to illustrate the advantages of SRTs and provide context regarding implementation and analysis. Section \ref{seq_time_pers} details three specific advantages of running SRTs. These advantages are exemplified by showing specific results from PERCS. We conclude by providing some practical recommendations for researchers designing their own SRTs in Section \ref{sec:implications-for-practice}.

\section{Prior Work}\label{sec:prior-work}

\subsection{Adaptive Interventions}

Adaptive interventions have been shown to be useful in SDLEs, and have been used extensively in web-based adaptive educational systems \cite{Brusilovsky_2003}. For instance, in \cite{Pardos_2017} learners were provided personalized content recommendations based on their clickstream data, and in \cite{Davis_2018b}, learners were provided personalized feedback on their learning plans. Adaptive sequences of interventions have also been developed in MOOCs, and \cite{David_2016} used adaptive sequencing for problems based on predictions of student knowledge acquisition. Similarly \cite{Davis_2018} chose quiz questions based on course content accessed previously by the learner. While these are only a few examples of adaptive interventions in large scale learning environments, they motivate our desire to improve the process by which such interventions are developed. 


In the work discussed, adaptive interventions were developed using learning theory and intention \cite{Davis_2018}, or prediction and machine learning \cite{Pardos_2017, Yu_2017, David_2016}.  In all examples, experimentation was not used to develop the adaptive intervention. In some cases \cite{Davis_2018, David_2016}, experimentation was used for evaluating the adaptive intervention. In these cases, an A/B test is used to compare the designed intervention to a control.
%In contrast, the overarching aim in SRTs is to use experimentation to decide how to best personalize and adapt an intervention. 

%SRTs do not optimize throughout the trial and can be thought of as pure exploration. See Section~\ref{sec:compare} for more details on these differences.

Reinforcement learning techniques, such as multi-armed bandits and contextual bandits, are a type of adaptive interventions which combine exploration (often done through implicit experimentation) and optimization. They use real-time data to learn how to adapt and have also been shown to be useful in SDLEs \cite{Liu_2014b, Clement_2013, Segal_2018, Rafferty_2018}.

\subsection{Experimental Designs}

Experimentation in SDLEs is a common tool for evaluating interventions. 
Unlike quasi- or natural experimental settings \citep[e.g.,][]{gonzalez_2015, Mullaney_2015}, by randomly assigning interventions, effects of interventions can be separated from effects of confounders (variables that relate both to the type of treatment received and to subsequent outcomes).

A/B tests are a valuable experimental design for improving content and evaluating interventions in MOOCs \cite{savi_2017}. In \cite{Renz_2016}, for example, A/B tests evaluated emails and course on-boarding to improve learner engagement and prevent dropout. In \cite{Davis_2016}, A/B tests were used to test the effectiveness of self-regulated learning strategies. Kizilcec and Brooks \cite{Kizilcec_2017} survey prior work utilizing A/B tests in MOOCs to evaluate nudge interventions and test theory-driven course content changes.


There has also been considerable work in other types of experimental designs beyond A/B testing in SDLEs. \textit{Factorial designs}  \citep[e.g.,][]{Lomas_2013} are common ways to evaluate multiple experimental factors simultaneously. 
%Factorial designs are still single-randomized trials, however, factorial designs can be incorporated into SRTs, as we demonstrate in the design of PERCS in Section \ref{sec:percs}. 
\textit{Automatic experimentation} \citep[e.g.,][]{Liu_2014}, where algorithms are used to search through different intervention options, is another alternative to A/B testing. Though automatic exploration of intervention options may be more efficient, intervention options are still evaluated with single-randomized trials. \textit{Adaptive experimental designs} change the randomization probabilities to favor efficacious treatment. With the goal of both evaluating treatment and helping learners currently in the trial \cite{Chow_2008}. Adaptive designs have been used in SDLEs \cite{Williams_2018}. We address the differences between SRTs and these other kinds of designs in Section \ref{sec:compare}.


\section{Sequential Randomized Trials} \label{sec:seqential-randomization}
\subsection{An Overview}

SRTs are trials where an individual is randomized multiple times throughout the course of the trial. Suppose there are two intervention options, such as learners receiving videos taught by a female instructor (intervention A) or a male instructor (intervention B). The simplest example of a SRT would be: During week 1, users have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B.  During week 2, users are re-randomized to another treatment. They again have a 50\% chance of receiving either intervention A or B, independent of their week 1 treatment or activity. Hence, about 25\% of users will have received one of each sequence (A, A), (A,B), (B,A), or (B,B), where the parenthetical notation means (week 1 treatment, week 2 treatment).

This simple SRT can be modified for both practical and scientific reasons. Common modifications include using different time durations (e.g., re-randomize every month), increasing the number of time points (e.g., each person is randomized 10 times instead of twice), changing the number of treatments (e.g., A vs B vs C instead of A vs B, or A vs B in week 1 and C vs D in week 2), and altering the randomization scheme (e.g., not having uniform randomization probabilities each week, or, in week 2, only re-randomizing inactive users).

Trials with sequential randomization \cite{Lavori_2004, Lavori_2000} have become relatively common in clinical settings \cite{Lei_2011} and are becoming more prevalent in educational settings \cite{almirall_2018}.  Two of the most common types of SRTs are Sequential Multiple Assignment Randomized Trials (SMARTs) \cite{Murphy_2005}, and Micro-randomized Trials (MRTs) \cite{Klasnja_2015}. In a prototypical SMART, individuals are first randomized to one of two different treatment options. Then, at a pre-specified decision point following initial intervention,  users who did not respond to initial treatment are re-randomized, while users who did respond to initial treatment are not re-randomized and continue with the efficacious initial treatment \cite{Pelham_2016}. MRTs have been mostly used in the mobile health space, where interventions (such as delivering reminders on a subject's phone) can be delivered quickly and frequently. Due to the high frequency of delivery, users in an MRT are typically re-randomized hundreds or thousands of times to identify when interventions should be delivered to maximize short-term impact.


\subsection{Comparisons to Other Designs}\label{sec:compare}

\subsubsection{A/B Testing}

SRTs are distinctive from many other types of common trial designs. In A/B tests (often called a 2-arm randomized controlled trial in healthcare and education), each subject is randomized \textbf{one time} to either intervention A or intervention B. SRTs randomize subjects several times, causing them to receive multiple treatments throughout the trial. Through sequential randomization, researchers can answer many more questions about sequencing, timing, and personalizing adaptive interventions, as described in Section~\ref{seq_time_pers}.

A/B tests can still be used to evaluate adaptive interventions. For example, if treatment A is defined as an adaptive intervention (e.g., a fixed sequence of different intervention options) and treatment B is defined as a control, an A/B test can compare the adaptive intervention to the control with a single randomization. Unfortunately, since randomization only occurs once, this trial is limited in answering questions about sequencing, timing, and personalizing.

A/B tests are often used in confirmatory trials. Confirmatory trials are trials used to ensure strong evidence (or additional evidence) of a treatment's efficacy, where one intervention is the treatment of interest and the other intervention is the control. Confirmatory trials differ from exploratory trials, which are typically done in the early stages of intervention development to help researchers narrow down intervention options, understand efficacious intervention components, and learn how individuals' characteristics change intervention efficacy. SRTs are specifically useful as an exploratory trial in SDLEs, with the goal being to leverage the large population of learners to explore a large number of possible treatment sequences, and learn how to adapt those sequences. After running a SRT and developing a high quality adaptive intervention, the designed intervention sequence can be confirmed in a simple A/B confirmatory trial where the proposed intervention sequence is compared to a control \cite{Collins_2007}.


\subsubsection{Online Optimization Designs}

There are other designs (both experimental and not) which aim to optimize intervention delivery while simultaneously collecting data. In adaptive trial designs \cite{Chow_2008}, randomization probabilities are changed throughout the trial in order to both provide efficacious treatment to users, and still obtain good estimates of treatment effects. 
Online reinforcement learning methods (such as multi-armed bandit and contextual bandit algorithms) can also be used for optimizing intervention delivery \cite{Liu_2014b, Clement_2013, Segal_2018, Rafferty_2018}. These online treatment optimization techniques can provide better treatment for new subjects (based on data from previous subjects) \cite{Williams_2018}, and can also provide better treatment for the same subject at a later time (based on the subject's earlier data) \cite{Clement_2013}.

SRTs are distinctive from adaptive trial designs and online reinforcement learning methods since they do not perform any online optimization. That is, SRTs do not use data collected throughout the trial to change randomization schemes. The randomization scheme is pre-specified and stationary. In reinforcement learning language, SRTs can be seen as pure exploration with no exploitation.

Even though a SRT is not explicitly aimed to benefit learners during the trial, there are advantages of not using earlier trial data to inform future treatment allocation:
\begin{enumerate}
\item Using online optimization techniques can cause bias in estimating treatment effects \cite{Nie_2017, Rafferty_2018}. Since data collected during the trial does not change a SRT's randomization scheme, issues of bias do not arise.

\item Many reinforcement learning methods require assumptions for good performance. In multi-armed bandits \cite{Liu_2014b, Clement_2013, Rafferty_2018} and contextual bandits \cite{Lan_2016}, for example, it is assumed that prior treatment does not change the efficacy of future treatment. This assumption may not be realistic. Since SRTs do not optimize, they do not require any assumptions about the data. Instead, they provide a rich data set useful for checking such assumptions and validating the eventual use of reinforcement learning methods.

\item SRTs provide rich exploratory data for discovering which variables are valuable for informing treatment decisions, making them useful when these variables are not known (see Section \ref{sec:personalization-with-srts}). In contrast, many reinforcement learning algorithms, such as contextual bandits \cite{Lan_2016}, require the context (i.e., learner characteristics informing treatment decisions) to be specified. 

\item SRTs can actually utilize reinforcement learning methods. Batch off-policy reinforcement learning algorithms (such as Q-learning) can be applied to SRT data to discover an optimal adaptive intervention, as in \cite{Zhao_2009}.
     
\end{enumerate}


%% old phrasing that's not right
%SRTs are different from adaptive trial designs. Data from a SRT informs the development interventions which are adaptive (i.e., interventions which change throughout the course for a given user), however, the trial itself is non-adaptive. Unlike adaptive trial designs, in SRTs all users are randomized the exact same way; the randomization of new users does not change based on data collected during the trial.

%Both trial designs are advantageous, but for different reasons. If research questions are about how to personalize, adapt, and sequence a series of interventions for an individual, SRTs should be used.  If a researcher's goal is to evaluate an intervention while also hoping to improve learning outcome for users currently in the trial, then they should use adaptive designs.
%There is some work on how adaptive designs can inform how to personalize interventions (using contextual bandit algorithms)[cite], however, personalization capabilities is limited compared to SRTs (see section blah).

%They are instead used to develop interventions which adapt.  
% and they adapt within a person.

\section{Applications of SRTs} \label{sec:srt_examples}


SRTs can inform a large variety of interventions including course content sequencing, course material manipulations, and learner nudges (such as encouraging messages and problem feedback). We highlight three examples. The first two examples are hypothetical scenarios to demonstrate different types of possible SRTs. The third example, PERCS, is a SRT run in a data science MOOC and is the main working example. 

\subsection{Video Optimization} For each video in an MOOC, there are two versions, one video which shows only slides and one which shows the instructor's head occasionally interspersed with the slides \cite{Guo_2014}. Researchers are unsure about which sequence of videos are better. 
Learners might prefer only slides, some might prefer those with instructors, or some might prefer a variety of videos. Also, there may be learner characteristics that affect learner preference. For example, learners who initially performed poorly after watching an instructor video might be better off seeing a slide-only video. To provide insight into these questions and hypotheses, a researcher could run a SRT: When a learner enters a course, they are randomized initially to receive an instructor video or a slide only video. Then, after watching the first video, they are re-randomized to either instructor or slide video for the next video they watch. This continues through the entire course.

\subsection{Content Spacing} Researchers are often unsure about optimal review problem sequencing to maximize knowledge retention while minimizing review time \cite{reynolds1964effects}.  Learners may benefit from frequent review at the beginning then less frequent review later. Secondly, how should learner characteristics inform review problem spacing? Should learners who are performing well receive different problem spacing sequences than poor performing learners?
A SRT can answer these questions: For a problem recommendation system, a learner starts the recommender for a time window (e.g., 50 problems). Then, after this time period, every learner is randomized to one of 3 groups: no review, minimal review, large review. The grouping determines how often they receive previously-seen problems (for review) during the next 20 problems. If a learner is in the no review, minimal review, or large review group they will receive previously-seen problems 0\%, 5\%, or 20\% of the time, respectively. After completing the next 20 problems, each user will be re-randomized to one of the 3 groups. This randomization scheme continues. Every 20 problems completed, a user is re-randomized to one of the 3 groups.

\subsection{Problem-based Email Reminder Study (PERCS)}\label{sec:percs}


\subsubsection{Motivation}
\label{sec:rqs}

A well-known challenge in MOOCs are the low completion rates. While there are many factors contributing to MOOC dropout \cite{Greene_2015}, the goal of PERCS is to determine whether dropout can be ameliorated by using weekly email reminders to motivate learners to engage with course content. Our context of inquiry was the [redacted for review] data science MOOC, taught by one of the authors. Weekly emails were sent to learners and may have contained one or more of several factors intending to impact learner engagement (see Table~\ref{tab:probs}):
\begin{enumerate}
    \item The email could have contained a motivating data science problem to challenge the user to learn the upcoming week's content. This factor was based on evidence from the problem-based learning literature suggesting that situating instruction in the context of problems is an effective way to engage learners \cite{barrows1985design}.
    \item  The email might also have contained a location specific primer and a data science problem relevant to that user's specific culture (e.g., an Indian user might receive a problem about Bollywood or weather patterns in India). This factor was based on the work in the culturally relevant and culturally responsive pedagogy communities, where situating instruction in a manner that considers the local context is seen as beneficial \cite{Aceves_2014a}.
    \item The email may have utilized growth mindset framing \cite{Dweck_2008}, a psychological framing method used to support learning. While growth mindset has been heavily studied, its effects are in dispute \cite{Kaijanaho_2018}, and growth mindset framing has seen only limited application in scaled online learning environments.
\end{enumerate}

Given these weekly email options, we hope to develop an adaptive intervention of weekly email reminders to increase engagement and reduce dropout. A high quality adaptive intervention should sequence emails in a way that promotes engagement continually through the course.  Since different emails may be more or less effective during different weeks in the course, each week, the intervention should send the most effective email for that week. Finally, since we might not expect the same email to work well for everyone, the intervention should also adapt to the learner's current course behavior. In order to develop a high quality adaptive intervention of emails, we need to answer the following research questions: 


\begin{enumerate}[label=RQ\arabic*]
    \item \textbf{Sequencing}: Which sequence of emails most improves course activity in later weeks?\label{rq1}
    \item \textbf{Timing}: Which email problem type is most effective, on average, for bringing learners back to the course during each week? \label{rq2}
    \item \textbf{Personalization}: Are certain data science problem emails more or less effective for active learners? \label{rq3}
\end{enumerate}
            
\subsubsection{Design}

\begin{figure}
    \centering
    \includegraphics[width= 0.7 \columnwidth]{img/email_structure_narrow_redacted.pdf}
    \caption{Example email structure using content which is populated based on their assigned treatments. (A) Identity activation prompt. (B) Culturally-relevant problem using data related to geographic identity. (C) Reminder to return to course. (D) Link to code for problem-based practice. (E) Growth mindset framing. (F) Link to problem solution. Elements of the same email type are grouped by color (see key).
    Learner, instructor, and course name redacted for review.}
    \label{fig:example-email}
\end{figure}

A sequentially randomized factorial trial design was an effective method to jointly address the main research questions of PERCS. At the end of weeks one, two, and three of the four-week long MOOC, learners were randomly assigned to receive one of four different email categories: an email message with a problem that reflects their geo-cultural situation based on IP address (\emph{cultural problem email}); an email with a generic, non-culture specific problem (\emph{global problem email}); an email with \emph{no problem}; or \emph{no email} at all. Those who received an email were uniformly randomly assigned to have the email be framed with or without growth mindset. 

The growth mindset factor crossed with the three email categories makes each week of PERCS a $2 \times 3$ factorial design with an additional control condition of no email. See Table~\ref{tab:probs} for each week's factorial design and randomization probabilities.


\begin{figure*}
    \centering
    \includegraphics[width = 0.8 \textwidth]{img/perts_design_trimmed.pdf}
    \caption{PERCS trial design. ``R'' indicates stages where randomization is conducted according to the probabilities in Table \ref{tab:probs}.}
    \label{fig:percs_design}
\end{figure*}

\begin{table*}[]
\begin{tabular}{ll|
>{\columncolor[HTML]{EFEFEF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |}
\cline{1-1} \cline{3-6}
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}No Email E_0} &  & Email E_1               & \cellcolor[HTML]{EFEFEF}No Problem Email (P_0) & \cellcolor[HTML]{EFEFEF}Global Problem Email (P_1) & \cellcolor[HTML]{EFEFEF}Cultural Problem Email (P_2) \\ \cline{1-1} \cline{3-6} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}0.14 (T_1)}   &  & No-Growth Mindset (G_0) & 0.14 (T_2)                                     & 0.14 (T_3)                                         & 0.14 (T_4)                                             \\ \cline{1-1} \cline{3-6} 
                                                           &  & Growth Mindset (G_1)    & 0.14 (T_5)                                     & 0.14 (T_6)                                         & 0.14 (T_7)                                             \\ \cline{3-6} 
\end{tabular}
\caption{An overview of the probability learners will be assigned to a treatment $T_n$. Individual treatments are shown in white cells, while groups of treatments are referred to by the tab row or column headers (e.g., all cultural problem emails as $P_2$)}
\label{tab:probs}
\end{table*}


Figure \ref{fig:example-email} illustrates an example email. The emails were developed in a ``cut and paste format'': When adding in a condition to an email (e.g., growth mindset framing or adding a problem), we do not change other aspects of the email, and simply insert text from the relevant condition into a consistent email template. Using the cut and paste across different conditions allowed us to attribute treatment effects purely to the condition being added, and not other aspects of the email. Emails are delivered directly using the Coursera platform's email capabilities for instructors.
 
The most novel aspect of PERCS is the sequential randomization. That is, a particular learner does not get randomized to a single email condition and remain in that treatment condition for all three weeks. Instead, as shown in Figure \ref{fig:percs_design}, each week, a learner is re-assigned (with the same randomization probabilities) to a different email condition. The randomizations across weeks are independent, hence in PERCS, there are $7^3$ ($343$) possible different email sequences students may receive.

\subsubsection{Notation}

Throughout the rest of the paper, we will be referring to specific treatments, groups of treatments, and sequences of treatments in PERCS. We introduce notation to ease our description. As shown in Table \ref{tab:probs}, $T_1, T_2, \dots, T_7$ refers to a particular email. For example, $T_2$ is an email containing no problem, and growth mindset framing. To refer to groups of emails, we used labeling contained in the column and row headers in Table \ref{tab:probs}. $E$ is used to group together conditions where any email was sent ($E_1$) vs no email being sent ($E_0$). So users in $E_1$ refer to any user receiving emails $T_2$ through $T_7$. $G$ is used to group together growth mindset emails ($G_1$) and non-growth mindset emails ($G_0$). Users in $G_0$ refer to any user receiving emails $T_5, T_6, $ or $ T_7$. $P$ is used to group together no problem emails ($P_0$), global problem emails ($P_1$), and cultural problem emails ($P_2$). Thus users in $P_1$ are are any users receiving emails $T_3$ or $T_6$.  Lastly, we use parenthetical notation to describe the sequences of emails over the three weeks, i.e., (week one treatment, week two treatment, week three treatment). As an example, we would refer to users who received a global problem email in week 1, any email in week two, and a no-growth mindset email in week three we use ($P_1, E_1, G_0$).


\subsubsection{Experimental Population}

We focused our trial on the two largest populations of learners enrolled in the course as determined by IP-address, Indian and US-based learners. All Indian and US learners who signed up for the [redacted for review] between the times of April 1, 2018 to June 10, 2018 participated in PERCS. A total of 8,681 unique learners (3,455 Indian, 5,226 US) were sent 22,073 emails. 
%% india 7717 3455
%% us 12,356 5,226

\subsubsection{A/B Testing Version of PERCS}

To highlight the advantages of sequential randomization, PERCS will be compared to the single-randomized, A/B testing version of PERCS (PERCS-AB). PERCS-AB has the exact same randomization probabilities as PERCS, however in PERCS-AB, prior to the start of week two, learners are randomized to one of the 7 email types, and are sent that exact same email type for the subsequent 3 weeks. Hence, there are only 7 possible sequences ($T_1, T_1, T_1)$, $(T_2,T_2,T_2)$, $\dots$,  $(T_7,T_7,T_7)$.


\section{Sequencing, Timing, and Personalizing Interventions through SRTs} \label{seq_time_pers}.
%or developing high quality adaptive interventiosn wtih srts

Next we highlight how SRTs can provide answers to questions regarding sequencing, timing, and personalizing interventions. For each type of question, we provide (1) an overview of the question and contextualize it within PERCS, (2) evidence of why SRTs are beneficial for answering that question as illustrated through comparing PERCS and PERCS-AB, (3) further discussion, and (4) answers to the question in the context of PERCS.

\subsection{Sequencing} \label{sec:optimal-sequence}

\subsubsection{Overview} 
When many different intervention options can be delivered at different times, proper sequencing of interventions is critical. An intervention that worked at one time, may not work at a later time. Also, receiving the same intervention multiple times may be less effective than receiving a variety of interventions. Researchers may not know which sequence of intervention options will lead to the best outcomes for learners. For PERCS, \ref{rq1} from Section~\ref{sec:rqs} refers to sequencing-- are there sequences of emails which improve course activity in the later weeks?

%\subsubsection{Research Questions}

%Research questions regarding effects of different treatment sequences include:

%For the \emph{Video Optimization} scenario we are interested in knowing throughout a course, whether learners prefer only videos with slides, only videos with instructors, or a variety. For the \emph{Content Spacing} scenario, we are interested in understanding whether learners will benefit from frequent review problems in either earlier or later time frames. Finally, for the \emph{PERCS} scenario we are interested in \ref{rq1} from Section~\ref{sec:rqs}, whether there are sequences of emails which improve course activity in the later weeks.

\subsubsection{Advantages of SRTs}

SRTs provide data that allows experimenters to compare different sequences of interventions. By re-randomizing learners, learners receive a variety of treatment sequences. In PERCS, for example, with the large sample size, there are learners who have the sequence $(T_1, T_1, T_1)$, $(T_1, T_1, T_2)$, $(T_1, T_2, T_2)$, or $(T_2, T_1, T_2)$. For the $7^3$ possible sequences of treatments, there are learners randomly assigned to each of those sequences.

By having learners randomized to all of these different sequences, researchers are now able to compare different sequences of treatment. For example, researchers could compare the effects on course activity of not receiving an email followed by two specific problem-based emails $(E_0, T_2, T_7)$ vs two different problem-based emails followed by not receiving an email ($T_3, T_4, E_0)$, by simply comparing the course activity of users randomized to these two sequences.

In A/B tests, since learners do not get re-randomized, sequence comparison can only be done for sequences where each learner received the same treatment the entire time. In PERCS-AB, learners are only randomized to 7 possible sequences and thus comparisons can only be done between these 7 sequences. If there was any benefit to receiving different interventions (and/or in a different order) then this could not be discovered by PERCS-AB. However one would note that all of the comparisons of PERCS-AB can be done with data collected through PERCS, coming at the cost of a reduced sample size. This tradeoff demonstrates again why SRTs are especially well situated for MOOC experimentation, where there is a large number of diverse participants (and thus a broad exploration might be suitable).
 
\subsubsection{Discussion}
%Comparing sequences of treatment groups

Often times, researchers are not interested in such specific sequence comparisons. Instead, they are interested in questions about sequences of groups of interventions. In this case, one could perform similar comparisons, but combining users over all of these groups. For example, in PERCS,
we can assess how often reminder emails should be sent. Is it better to space emails out weekly or bi-weekly?
%\footnote{Due to space limitations we do not describe the results here, and focus only on sharing the main RQs described in Section \ref{sec:rqs}. SRTs provide significant opportunity for broad experimental inquiry!}
To answer this question, we could compare course activity of users receiving the sequence which spaces emails out by 2-weeks $(E_1, E_0, E_1)$, to the sequence which sends emails every week $(E_1, E_1, E_1)$. The sample size for this comparison will be much larger than for the single sequence comparisons.

In addition to comparing groups of sequences, researchers might only be interested in comparing sequences for a small number of time points. For example, we could use data collected in PERCS to understand if the effects of week two problem-based emails on course activity were different based on what type of problem-based email the user had received in week one. Specifically, does getting no email vs cultural problem-based email in week one change the benefits of receiving a cultural problem email in week two?  To answer this question, we compare course activity in week two of users receiving sequences $(E_0, P_2, $any) vs ($P_2, P_2, $any). Notice we are not concerned with anything occurring in week three, so we include sequences with any treatment in week three (i.e., any includes $T_1, T_2, \dots, T_7$)

%In PERCS-AB, learners are only randomized to 7 possible sequences $(T_1, T_1, T_1), (T_2,T_2,T_2), \dots,  (T_7,T_7,T_7)$. Hence, comparisons can only be done between these 7 sequences. If there was any benefit to receiving different interventions, in a different order, this could not be discovered by PERCS-AB. Notice also that all of the comparisons of PERCS-AB can be done with data collected through PERCS, though this comes at the cost of a reduced sample size. This tradeoff demonstrations again why SRTs are especially well situated for MOOC experimentation.



\subsubsection{Results from PERCS} \label{results_seq}
We now present results answering \ref{rq1}. Since there are a large number of potential sequences, here we focus on the highest-level comparison, i.e., understanding the proper sequence of any email and no email. To do the comparison we look at the proportion of students returning to the course in week 4 (the final week) after receiving a given sequence of emails ($E_1$) and no email ($E_0$), as shown in Figure \ref{fig:seq_results}.

\begin{figure}
\includegraphics[width= \columnwidth]{img/seq.png}
\caption{95\% confidence intervals for the proportion of students returning to the course in week 4 after receiving a given three week sequence of emails ($E_1$) and no email ($E_0$)} \label{fig:seq_results}
\end{figure} 

We note some important observations. For US learners, sequences with emails sent in the first week (e.g.,those sequences which start with $E_1$, the last four columns in Figure \ref{fig:seq_results}), tend to be more beneficial than sequences without. For Indian learners this is not true. 
%and relative to US-based learners Indian learners perform the same or better in conditions where there was not an email sent in the first week (i.e., beginning with $E_0$) and worse in those conditions where there was an email in the first week (i.e., beginning with $E_1$). 
Overall, for both countries, the confidence intervals across sequences are mostly overlapping, indicating that differences in effects of various email sequences are not strongly significant. The size of the confidence intervals change due to the probability of receiving an email ($E_1$) being larger than the probability of not receiving an email ($E_0$).

%Notice also how the size of confidence interval changes based on the number of learners randomized to that group. The sequence of 3 weeks of no emails, $(E_0, E_0, E_0)$ only had a $(\frac{1}{7})^3$ chance of randomization while the sequence of 3 weeks of emails $(E_1, E_1, E_1)$ had a  $(\frac{6}{7})^3$ probability. If this sequence comparison was the primary aim of PERCS, randomization probabilities should change to give more balance across these sequences.

%For PERCS, we were most interested in understanding how to best sequence and space out emails with problems and emails without problems (RQ\ref{rq1}). We were not sure if users would be motivated by only problem-based emails, no-problem email reminders, or no emails at all.  Specifically, we were interested in understanding the sequential differences between the groups: 1) no emails ($E_0$), 2) no problem emails ($P_0$), 3) global problem emails ($P_1$), and 4) cultural problem emails ($P_2$) . Each week, a user could have received one of these four types of emails, providing $4^3$ = 64 sequences to compare (i.e., $(E_0,E_0,E_0), (E_0,E_0,P_0), (E_0,E_0,P_1), \dots (P_2,P_2,P_2)$). For users in each of these sequences, we create a confidence interval for the log number of course clicks throughout the entire course. The results are in table blah

\subsection{Timing}\label{sec:avg-treatment-effects}

\subsubsection{Overview}

Instead of being interested in a sequence of interventions, researchers might want to know about the effect of an intervention option at a particular time point. A treatment that was effective at the beginning of the course may be less effective towards the end of the course. By understanding effects of intervention options at a time point, designers can build adaptive interventions which deliver the optimal treatment at all times. For PERCS, \ref{rq2} from Section~\ref{sec:rqs} regards timing-- which email type is most effective during each week?

%\subsubsection{Research Questions}

%Research questions regarding treatment effects at particular time points include:

%\begin{itemize}
%\item \textbf{Video Optimization}: For the last video in the course, is it better to have the video contain slides only or to also feature the instructor?
%\item \textbf{Content Spacing}: What is the effect of frequent review (compared to no review) during the third set of recommended problems? 
%\item \textbf{PERCS}: Research question \ref{rq2} regards treatment timing.
%\end{itemize}

\subsubsection{Advantages of SRTs}


%For the last video in the course, is it better to have the video contain slides only or to also feature the instructor?
%What is the effect of frequent review (compared to no review) during the third set of recommended problems? 
%How does sending a cultural problem emails in week two effect the subsequent week's course activity, compared to not sending any email?

Answering research questions about treatment timing is done by estimating average treatment effects, i.e., the average effect of a given treatment option at a given time point. Here, the averaging is over all prior treatment received, allowing the effect to be only for the particular time point of interest.

SRTs permit the estimation of average treatment effects at various time points. By re-randomizing individuals, we can separately estimate average treatment effects at each time point and eliminate confounding with treatment delivered previously. In A/B tests, such a comparison is only possible the first time treatment is delivered. At times after the first treatment delivery, because the learner will have received the same treatment at all previous time points, the effect of a given treatment option is confounded with the effects of prior treatment.

To exemplify, in PERCS, to understand which email type is most effective in week 3, we compare the average effect of cultural problem emails in week 3 (any, any, $P_2$) compared to no email in week 3 (any, any, $E_0$). By doing this comparison, we average over all treatments delivered prior to week 3, and isolate the effect of interest to emails only in week 3. In PERCS-AB, such a comparison is impossible. We could only estimate the effects of cultural problem emails for all 3 weeks, to no email for all 3 weeks, ($P_2$, $P_2$, $P_2$) vs ($E_0$, $E_0$, $E_0$). The estimate in PERCS-AB is a compounding effect of cultural problem emails for all 3 weeks vs no email for all 3 weeks, instead of an average effect isolated to week 3.

In SRTs, average treatment effects can also be estimated for outcomes measured \textit{after} the next re-randomization (sometimes called delayed effects).  For example, in addition to understanding the average effect of cultural problem emails in week 2, on week 3 course activity in PERCS, we are also able to understand the average effect of cultural problem emails in week 2, on week 4 course activity (and other outcomes such as course completion). We do so by averaging over both week 1 treatment and week 3 treatment. This delayed effect cannot be estimated in PERCS-AB since, with no re-randomization after week 2, the estimate will be confounded by treatment in week 3.

\subsubsection{Discussion}
%The Difference Between Average Treatment Effects and Sequence Effects

%% I might be able to cut this

Research questions on average treatment effects often seem similar to questions regarding sequence effects. In order to elucidate the differences, below are 3 types of research questions in PERCS:
\begin{enumerate}
    \item What is the effect of a cultural problem email in week three, after not receiving any email prior? Compare ($E_0, E_0, P_2$) vs ($E_0, E_0, E_0$) \label{timing_rq1}
    
    \item What is the average effect of a cultural problem email in week three (averaging over all prior treatment)? Compare (any, any, $P_2$) vs (any, any, $E_0$) \label{timing_rq2}
    
    \item What is the effect of getting a cultural problem email every week until week three? Compare $(P_2, P_2, P_2)$  vs $(E_0, E_0, E_0)$ \label{timing_rq3}
\end{enumerate}

Questions \ref{timing_rq1} and \ref{timing_rq3} are questions of comparing sequences of treatments, while question \ref{timing_rq2} is about average treatment effects. Note that all three questions can be answered by PERCS, but only question \ref{timing_rq3} can be answered by PERCS-AB.

Also, one advantage of analyzing average treatment effects is that the sample size is typically larger than when comparing individual sequences of treatments, since the comparison does not restrict users based on what they received before or after the given week of interest.

\subsubsection{Results from PERCS}

To assess \ref{rq2}, for each week, we perform logistic regression with a binary outcome indicating whether the user clicks anything in the course during the week after receiving an email. The results are in Figure~\ref{avg_eff_results}. Negative values indicate a reduced chance of returning to the course, compared to no email, while positive values indicate an increased chance of returning to the course.

\begin{figure}
\includegraphics[width= \columnwidth]{img/average.png}
\caption{95\% confidence intervals of the log odds ratios of probability of returning to the course in the subsequent week for emails containing no problem, a global problem, or a cultural problem, when compared to being sent no email. {\large*} indicates a moderate effect with significance at $\alpha$ = .2}
\label{avg_eff_results}
\end{figure} 

The results in Figure~\ref{avg_eff_results} show that the impact of emails on Indian learners in weeks 2 and 3 is largely positive, but the impact of receiving a no problem email ($P_0$) is as good or better than receiving either global or cultural problem emails ($P_1$ and $P_2$, respectively). Also, in week 2, emails of all types were moderately effective, indicating this is a good time to send Indian users email reminders for this course.%, but including motivating data science problems in those emails may not be worth the effort.

For US learners, the effects are non-significant across all emails except for the cultural problem email ($P_2$) in the last week of the course, and the log odds ratios are small and in many cases negative. This indicates that for all weeks, emails for US users did not impact their propensity to return to the course, and may even deter them from returning -- a counterintuitive, but important, insight from PERCS regarding timing of communication with learners.

\subsection{Personalizing}\label{sec:personalization-with-srts}

\subsubsection{Overview}
%\TN{This should match beginning}
SDLEs are notable for the high degree of diversity both across and within learners \cite{Kizilcec_2013,Kizilcec_2017}. Due to this diversity, we might expect intervention effectiveness to vary along with relevant learner attributes. If an intervention works for a specific user at a given time, that intervention may not be effective for a different user, or even the same user at a different time.  Personalizing treatment, by discovering when and for whom certain treatments are most effective, is critical. For PERCS, \ref{rq3} from Section~\ref{sec:rqs} regards personalization-- are certain emails more effective for active learners?

In clinical trials, learning how to personalize treatment is synonymous with discovering \emph{moderators} \cite{Kraemer_2002}. Moderators are subject-specific variables which change the efficacy of an intervention. For example, if a MOOC intervention works better for older users than younger users, then age is a moderator and can then be used to personalize the intervention; one may deliver the intervention to older learners. Answering \ref{rq3} in PERCS is equivalent to understanding if previous course activity is a moderator of email effectiveness.
%
%\subsubsection{Research Questions}
%
%Research questions about moderator discovery for treatment personalization include:
%
%\begin{itemize}
%\item \textbf{Video Optimization}: If a learner watched a slide only video and then performed poorly, should they now be shown videos featuring the instructor?
%\item \textbf{Content Spacing}:  Do learners who are performing well throughout the course need to receive different review problem spacing sequences than poor performing learners? 
%\item \textbf{PERCS}: Research question \ref{rq3} regards treatment personalization.
%\end{itemize}
\subsubsection{Advantages of SRTs}

Some moderators can be discovered using A/B trials, however, SRTs permit the discovery of two other types of moderators: baseline moderators for additional sequences and mid-course moderators.

%Add jjw cite on personalization with RL - talk about how it can discover things to personalize on, not prespecify
\textbf{Baseline sequence moderators.} Baseline variables are measured prior to the first treatment randomization. Baseline variables include learner demographics (e.g., gender, location, age) and course activity measured prior to the first randomization (e.g., whether the users has taken the course previously, scores on early assignments, survey responses at the beginning of the course). Often these variables moderate the effect of treatments and can be used for personalization. Discovering baseline moderators helps understand how to personalize interventions to account for diversity across learners.

SRTs and A/B tests both permit the discovery of baseline moderators. However, in SRTs, because users receive a larger variety of intervention sequences (see Section \ref{sec:optimal-sequence}), this permits the discovery of baseline moderators for effects of each of these sequences. This leads to a richer and more specific understanding of the moderating effects of various learner characteristics.  For example, unlike PERCS-AB, we can evaluate how a learner's location moderates the effect of each email sequence analyzed in Section~\ref{results_seq}

%As an example, in both PERCS and PERCS-AB, one could answer the question: is the effect of 3 weeks of cultural problem emails different for Indian learners compared to US learners? However, in PERCS, one is able to evaluate the moderation of learners' location on a larger variety of treatment sequence comparisons. Indeed, the PERCS design allows an experimenter to evaluate the moderation of location on every possible sequence of interventions in the trial.  One could also answer questions about how location moderates treatment sequence efficacy: is the effect of sequences which vary cultural and global problem emails different for Indian learners compared to US learners? PERCS-AB is not able to answer this second question since no users are re-randomized to receive both cultural and global emails throughout the course. PERCS-AB is only able to evaluate moderation of baseline variables on the small number of sequences in the trial.

%% Could put in examples from other example trials here if it warrants more explanation
\textbf{Mid-course Moderators.} Baseline moderators are important for personalizing initial treatment (or treatment sequences), however, understanding how to change treatment based on variables measured throughout the course -- mid-course moderators -- is critical. Discovering mid-course moderators tells practitioners how to personalize interventions throughout the course to account for heterogeneity both across different users and within a user over time. 

Unlike A/B tests, SRTs permit the discovery of mid-course moderators. Statistically, due to bias introduced when including post-randomization variables in analyses, one can only discover moderator variables measured prior to randomization \cite{Kraemer_2002}. If all learners were only randomized once, potential moderators measured after the first treatment cannot be discovered. By re-randomizing in SRTs, moderators measured before each of the randomizations (which now includes mid-course data) can be discovered. 

%<Should I further explain here the specifics, like I still have to preserve ordering, I can only assess there moderation on future treatment>

%Are certain data science problem emails more or less effective for active learners?

%we hypothesized that growth mindset framing in emails sent at the end of week three only works well for students who were inactive during week 3, because they would benefit from the growth mindset encouragement. Because users were randomized again at the end of week 3, we can use PERCS data to assess how week 3 activity moderates the effect of growth mindset emails (sent at the end week 3) on week 4 activity. In PERCS-AB, week three course activity cannot be assessed as a moderator in PERCS-AB since it was measured after the one and only randomization in week one. 

Because users were randomized again at the end of week three, to answer \ref{rq3} about emails sent during week three, we can use PERCS data to assess how activity during week three moderates the effect of data science problem emails (sent at the end week three) on week four activity. In PERCS-AB, week three course activity cannot be assessed as a moderator since it is measured after the one and only randomization in week one. 

\subsubsection{Discussion}

We can also evaluate mid-course moderators that include previous treatment. For example, we may think that responsiveness to previous treatment could inform how to personalize future treatment. Those that were responsive should continue getting the same treatment while those that were non-responsive should get assigned different treatment. In PERCS, for example, we might expect week two emails to benefit users who responded positively to emails in week one. One could assess this by comparing two groups: Group 1 are users who received an email ($E_1$) but did not click in the course afterwards (i.e., email non-responders). Group 2 are users who received an email ($E_1$) but did click in the course afterwards (i.e., email responders). We could compare the effect of emails in week two for Group 1 vs Group 2.


%In PERCS, we hypothesized that growth mindset emails are more effective for users indicating they liked growth mindset in the previous week and users indicating they did not like non-growth mindset in the previous week. More specifically, there are four groups of learners: Group 1 are learners who received growth mindset framing in week one and had course activity in week two (i.e., growth mindset responders), Group 2 are learners who received growth mindset framing in week one and had no course activity in week two (i.e., growth mindset non-responders), Group 3 are learners who received no growth mindset framing in week one and had course activity in week two (i.e., no growth mindset responders), Group 4 are learners who received no growth mindset framing in week one and had no course activity in week two (i.e., no growth mindset non-responders). We expected growth mindset framing in week two emails to benefit Groups 1 and 4 more than Groups 2 and 3. By re-randomizing at the end of week two, we assess moderation by comparing treatment effects of growth mindset framing in week two emails for Groups 1 and 4 vs Groups 2 and 3.

Discovering how to personalize based on mid-course activity is one of the major benefits of SRTs. These discoveries allow educators to select interventions that meet the needs of learners as they transition throughout the course. Also, as learning content optimization starts to happen in real-time (i.e., reinforcement learning), knowing which real-time variables to measure and use for online optimization is critical. SRTs permit this discovery.

%\TN{sentence like this here but for within leaners: Discovering baseline moderators helps understand how to personalize interventions to account for heterogeneity between different learners.}

\subsubsection{Results from PERCS}

\begin{figure}
\includegraphics[width = \columnwidth]{img/moderator_plot.png}
\caption{95\% confidence intervals of the log odds ratios of probability of returning to the course in the subsequent week for emails containing no problem, a global problem, or a cultural problem, when compared to being sent no email, The log odds ratio is calculated for users who had activity (active) or did not have activity (inactive) in the prior week.} \label{fig:moderator}
\end{figure}

For PERCS, we were most interested in previous week's course activity as a mid-course moderator. We wanted to see how different types of emails effect active and inactive users differently. Active users are defined as users who had one or more clicks in the course during the previous week. Before the trial, we did not know if problem-based emails would encourage inactive users (because they need the motivational reminder) or discourage inactive users (because the problem may be too advanced). To assess this, in Figure~\ref{fig:moderator} we plot the log odds ratios of the probability of returning to the course in the subsequent week for different emails conditions, compared to the control of no email. A positive log odds ratio indicates users had a higher chance of returning to the course after receiving the corresponding email problem type (compared to the no email control).

%There are two key observations drawn from the results in 
In week one, for both US and Indian learners, reminder emails of all types performed better for active users than inactive users (higher log odds for blue than magenta, Figure~\ref{fig:moderator}). In week three, the sign of the moderation switched, as emails performed better for inactive users compared to active users (higher log odds for magenta than blue). The difference was larger for Indian learners. Also, the log odds ratios for inactive users were positive, while the log odds ratios for active users were negative. To ensure we encourage inactive users to return to the course while not discouraging active users, email sending should adapt based on both users' previous course activity and the course week.

\section{Implications for Practice}\label{sec:implications-for-practice}

This section outlines some useful considerations for researchers who are interested in designing and running SRTs for SDLEs. First, before thinking about trial specifics, researchers should always remember that experiments are created to inform scientific understanding and answer questions about interventions. Deciding if a SRT is the correct trial design depends purely upon the scientific questions of interest. For example, if researchers are not interested in understanding how to sequence, time, and personalize interventions, running a SRT is unnecessary. In PERCS, if a researcher were interested in only comparing two sequences of interventions then it may be best to run an A/B test on those two sequences and forgo answers to other questions. 

In situations where a SRT is appropriate, there are also important trial design considerations.  All intervention sequences in a SRT should be useful, feasible, and scalable. It is useless to evaluate intervention sequences which could never be done in practice or which are knowingly deleterious to subjects. For example, suppose a researcher was curious about optimal ordering of course content and, in turn, sequentially randomized learners to various sequences of content. If content B requires information taught in content A, none of the sequences in the experiment should place content B before content A. As another example, in PERCS, because the MOOC platform does not currently support fully-automated, scheduled delivery of email, messages were only sent once per week. We did not explore the possibility of sending emails many times per week (e.g., re-randomizing email sending every day) because, in practice, interventions which require manual daily email sending would not currently be feasible for instructors on this platform.

As in any other trial design, sample size and power calculations are important for SRTs. Sample size calculations should be based off of the most important research questions the trial intends to answer. Since there are a larger number of possible treatment sequences in a SRT, calculating power and sample size requires researchers to consider which subset of users will be randomized to the sequences of interest. Then, sample size calculations are similar to A/B tests for both comparing interventions and discovering moderators \cite{Oetting_2011}. 
Due to the larger space of potential treatment sequences, sample sizes usually need to be larger for SRTs (compared to A/B tests). To increase power, researchers may consider changing randomization probabilities to favor interventions of interest. 
%For example, in PERCS, if our primary interest was in comparing cultural problem emails to global problem emails, we might change the weekly randomization probabilities in Table \ref{tab:probs} to favor these two interventions.



\section{Discussion}

Adapting, sequencing, and personalizing interventions is critical to meet the diverse needs of learners in SDLEs. When designing adaptive interventions, experimentation is useful for evaluating and comparing possible sequences. Unfortunately, single-randomized A/B tests cannot answer questions about ways to adapt and sequence interventions throughout a course.  In this work, we demonstrated how a new type of experimental design, SRTs, are valuable for developing adaptive personalized interventions in SDLEs. SRTs provide answers to questions regarding treatment sequencing, timing, and personalization throughout a course. Answers to these questions will both improve outcomes for learners and deepen understanding of learning science in scalable environments.

In this work, we provided a few examples of different SRTs. There are many more variations of SRTs that are useful for answering additional research questions. In PERCS, all users have the same randomization for all three weeks. However, if a certain learner is evidently responding well to treatment, it may not make sense to re-randomize them and change their current treatment. Many Sequential Multiple Assignment Randomized Trials (SMARTs) \cite{Murphy_2005, Pelham_2016} solve this issue by varying second stage randomizations based on a subject's response to prior treatment. This design is useful when moderators are known beforehand. It's important to note that these changes in randomization are pre-specified and intended for exploring adaptive interventions, not online optimization.

Other variations of SRTs may be useful to answer research questions in SDLEs. Since many online courses are accessible to learners at any time, randomization timing could be based on when each user enters the course (randomized one, two, and three weeks from the day the user enrolls in a course). If treatment delivery timing is a research question, the delivery time can also be (re)randomized (i.e., each week of the course, re-randomize users to receive one weekly email or seven daily email reminders). Also, since many SDLEs provide learners with all course content at the beginning of the course, a trial aiming to re-randomize course content could use trigger-based re-randomizations--where users' future content is only changed after they have watched a certain video or completed a particular assignment--to prevent early exposure to future treatment.

%In addition to content access, SDLEs have other unique aspects. In online courses, users can often enter an online course at any time.  In an A/B test, if randomization to treatment occurs during the course start date, users enrolled after that date will not be used in the study. In SRTs, since users will be randomized again at later times, the late enrolling students could potentially be used in these later randomizations. However, thoughtful analysis and statistical methodology needs to be developed to ensure proper estimation of treatment effects.

Though useful, SRTs have limitations. SRTs are non-adaptive trial designs. If an experimenter wishes to both learn efficacious treatments and provide benefit to learners in the current trial, adaptive designs such as \cite{Williams_2018} would be more appropriate. Combining adaptive designs with SRTs may also be useful for both developing high-quality adaptive interventions and improving benefits for current learners \cite{Cheung_2015}.

PERCS also had some limitations. For one, during our first iteration of the trial, the emails contained syntax errors, and some treatment groups did not receive emails. These errors were fixed for future iterations and the error-free iterations were the ones used in our analysis. Secondly, since some users (10\%) retook the online course multiple times, those users were repeated in multiple iterations of the trial. Lastly, it's important to note that PERCS was an exploratory trial not a confirmatory trial. The goal of PERCS was to explore several sequences of treatments and evaluate their efficacy for different learners. The next step for PERCS is to narrow down best treatment options based on current data (which may be different for Indian and US learners). Since the current evidence is not extremely strong, we would then run a second SRT with fewer treatments, acquiring more data on those treatments of interest. Once we have enough evidence to suggest which sequence of emails is optimal, we can then compare this learned optimal sequence of emails to a control in an A/B test confirmatory trial. Treatment A would be the hypothesized optimal adaptive sequence of emails and treatment B would be no email.



%\pagebreak
%\pagebreak

%\subsection{nonsense}

%


==> nonsense-body-from-before.tex <==
% after this it's all poo
Sequential randomization refers to the randomization of an individual multiple times throughout the course of the trial. Suppose there are two types of interventions, intervention A and intervention B. The simplest example of a sequentially randomized experiment would be: During week 1, users have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B.  During week 2 users are re-randomized to another treatment. They again have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B, independent of what happened in week 1. Hence, about 25\% of users will have received each sequence (A, A), (A,B), (B,A), (B,B), where the parenthetical notation means (week 1 treatment, week 2 treatment).

This simple sequential randomization scheme can be modified for practical and scientific reasons. Common modifications include using different time durations (e.g., re-randomize every month), increasing the number of time points (e.g., each person is randomized 10 times instead of twice), changing the number of treatments (e.g., A vs B vs C instead of A vs B, or A vs B in week 1 and C vs D in week 2), altering the randomization scheme (e.g., not having 50/50 randomization probabilities each week, or, in week 2, only re-randomizing inactive users).

Sequential randomization schemes have become relatively common in clinical settings [cites] and are becoming more prevalent in education settings [cites].  Two of the most common types of sequential randomization schemes are Sequential Multiple Assignment Randomized Trials (SMARTs) [cite Susan?s paper], and Micro-randomized Trials (MRTs) [cite Pedja?s paper]. SMART designs typically involve two randomizations, and often, the second randomization is different for different users. For example, users who didn?t respond to treatment after randomization 1 may be re-randomized, while users who did respond to treatment after randomization 1 are not re-randomized and continue with the efficacious initial treatment [cite SMART with this design]. MRTs have been mostly used in the mobile health space, where interventions (such as delivering reminders on your phone) can be delivered quickly and frequently. Because of the high frequency of interventions, MRTs are unique because they usually involve hundreds or thousand of re-randomizations.

\subsection{Comparisons to other trial designs}

Sequentially randomized trials are distinctive from many other types of common trial designs. In a typical A/B test (often called a 2-arm randomized control trial in healthcare and education), subjects are randomized one time to either intervention A or intervention B, and receive that same treatment for the entire length of the study.
http://ceur-ws.org/Vol-1688/paper-19.pdf

Sequentially randomized trials sometimes gets confused with adaptive trial designs. Adaptive trial designs are trial designs where An example of an adaptive trial design is a ?play the winner? or bandit type trial designs where, based on initial trial data collected from users, new users have different randomization probabilities which favor efficacious treatment. Another example of adaptively adjusting experimental conditions mid-trial. If intervention A starts to look much better than intervention B, then intervention B is dropped in future users? randomizations and a new intervention (B*) will be introduced.

Sequentially randomized trials are different from adaptive trial designs because in sequentially randomized trials, all users are randomized the exact same way. The randomization of new users does not change based on data collected on previous users.  Adaptive trial designs attempt to perform exploration and optimization of interventions simultaneously during the trial. Sequentially randomized trials, on the other hand, do not do any mid trial optimization. They produce a batch data set which can then be analyzed (post-trial) to understand how to optimize interventions and intervention sequences.

There are trial designs which combine sequential randomization with adaptive trial designs. Future randomizations for a particular user may change based on evidence from initial randomizations.
However, for simplicity, all of the sequentially randomized trials in this work will assume that all individuals undergo the exact same randomization scheme. 

Confirmatory trials are trials used to ensure strong evidence (or additional evidence) of a treatment?s efficacy. Confirmatory trials are typically single-randomized A/B tests where one intervention is the treatment of interest and the other intervention is the control. Confirmatory trials differ from exploratory trials. Exploratory trials are typically done in the early stages of intervention development to help researchers narrow down intervention options, understand efficacious intervention components, and learn how individuals? characteristics change intervention efficacy. Sequential randomization are useful as an exploratory trial. The goal is to explore a large number of possible treatment sequences, and learn how to personalize and optimize those sequences. After running a sequential randomized trial and designing an optimized sequence of interventions, the designed intervention sequence can be confirmed in a simple A/B confirmatory trial where the proposed intervention sequence is compared to a control.



\subsection{Applications of sequential randomization in MOOCs}

In this section I discuss a bunch of potential applications and possible interventions that could be evaluated using sequential randomization. See meeting 9/11/18 for examples.

Next, we provide a detailed example of the first-ever sequentially randomized experiment run in a MOOC, the Problem-based Email Reminder Coursera Study.


\subsection{Problem-based Email Reminder Coursera Study (PERCS)}

\subsubsection{Motivation behind PERCS}

A well-known challenge in MOOCs is low completion rates. While there are many factors contributing to MOOC dropout, the goal of PERCS was to see if dropout could be ameliorated by using weekly email reminders to motivate learners to engage with course content. These emails potentially contained a few factors intending to impact learner engagement. The email could contain a motivating data science problem to challenge the user to learn the upcoming week?s content. The email  might also contain a location specific primer and a data science problem relevant to that user?s specific culture (e.g., an Indian user might receive a problem about Bollywood or weather pattern in India). Lastly, the email may utilize growth mindset framing, a psychological framing method used to support learning.  See Table 1 for an overview of all the different kinds of emails.
 
Given all these different types of possible emails, the main research questions (ordered based on priority) were:
1. Which sequence of emails causes the highest rate of completion?
2. Which type of data science problem email (no email, no problem, generic data science problem, or culturally relevant data science problem) is most effective for bringing learners back to the course?
3. Are certain data science problem emails more or less effective for active learners?        
4.Does growth mindset framing improve an emails ability to bring learners back to the course?

\subsubsection{Design of PERCS}

A sequentially randomized factorial trial design was an effective method to jointly address the main research questions of PERCS.  At the end of weeks one, two, and three of the four-week long MOOC, learners were randomly assigned to receive one of four different email categories: an email message with a problem that reflects their geo-cultural situation based on IP address analysis (personalized problem condition), an email with a generic non-culture specific problem (global problem condition), an email with no problem (no problem condition), or no email at all (no email condition). These learners were also randomly assigned to have their email be framed with a growth mindset or without a growth mindset. The growth mindset piece crossed with the three email categories makes each week of PERCS a 2x3 factorial design with an additional control condition of no email. See table 1 for each week?s factorial design and randomization probabilities.
 
The most novel aspect of PERCS is the sequential randomization. That is, a particular learner does not get randomized to one email condition and remain in that treatment condition for all 3 weeks (as is typically done in experiments). Instead, each week, a learner is re-assigned (with the same randomization probabilities) to a different email condition. The randomizations across weeks are independent. Hence, in PERCS, there are $7^3$ possible trajectories of emails, for example, (A,A,A) (A,B,C) (A, A, G), where where the parenthetical notation means (week 1 treatment, week 2 treatment, week 3 treatment) with letters corresponding to treatment in Table 1.

\subsubsection{Participation in PERCS}

All learners who signed up for the Introduction to Applied Data Science with Python course on Coursera between the times of April 1, 2018 to June 10, 2018 participated in PERCS. A total of 15,037 unique learners were sent 28,446 emails. 

\subsubsection{AB Testing Version of PERCS}

To highlight the advantages of sequential randomization within PERCS, PERCS will be compared to the single-randomized, AB testing version of PERCS (called PERCS-AB). PERCS-AB has the exact same randomization probabilities as PERCS, however in PERCS-AB, prior to the start of week two, learners are randomized to one of the 7 email types, and are sent that exact same email type for the subsequent 3 weeks. Hence, there are only 7 possible trajectories (A, A, A), (B,B,B) ?, (G,G,G).

\section{Discovering an optimal sequence of treatments}
Is it better to space out review problems by?? 
For PERCSs, which sequence of emails (and no emails) leads to most returns to the course?
All of these questions are asking about optimizing and comparing sequences of interventions.

Sequentially randomized trials provide data that allows experimenters to compare different sequences of interventions. By re-randomizing learners, learners receive a variety of treatment sequences. In PERCS, for example, with the large sample size, there are learners who have the trajectory (A, A, A), (A, A, B), (A, B, B), (B, A, B), etc. For the $7^3$ possible sequences of treatments, there are learners randomly assigned to each of those sequences.

By having learners randomized to all of these different trajectories, researchers are now able to compare different sequences of treatment. For example, researchers could compare the effects on course activity of (No email, No problem growth mindset email, Culturally personalized non-growth mindset email) to (Global problem growth mindset email, Culturally personalized growth mindset email, No email), by simply comparing the course activity of users randomized to these 2 sequences.

Often times, researcher are not interested in such specific sequence comparisons. Instead, they are interested in questions about sequences of groups of interventions. In this case, one could perform similar comparisons, but combining users over all of these groups. For example, in PERCS, we were curious about how often reminder emails should be sent. Is it better to space emails out weekly or bi-weekly? To answer this question, we could compare course activity of users under the sequence ({B, C, D, E, F, G}, {A}, {B-G}), i.e., the trajectory which spaces emails out by 2-weeks, to (B + C + D + E + F + G, B + C + D + E + F + G, B + C + D + E + F + G), i.e., the trajectory which sends emails every week.  The sample size for this comparison will be much larger than for the single sequence comparisons.

In addition to comparing groups of sequences, researchers might only be interested in comparing sequences for a small number of time points. For example, in PERCS, we were curious if the effects of week two 2 problem-based emails on course activity were different based on what type of problem based email the user had received in week one1. Specifically, does getting no email vs no problem email vs problem based email in week one1 change the benefits of problem-based emails in week 2?  To answer this question, we compare course activity in week 2 of users receiving sequences (A, D + E + F + G, all), (B + C, D + E + F + G, all), and (D + E + F + G, D + E + F + G, all). Notice how we were not concerned with anything occurring in week three3, so we include sequences with any email in week three3.

In PERCS-AB, learners are only randomized to 7 possible trajectories (A, A, A), (B,B,B) ?, (G,G,G). Hence, comparisons can only be done between these 7 trajectories. If there was any benefit to receiving different interventions, in a different order, this could not be discovered by PERCS-AB. Notice also that all of the comparisons of PERCS-AB cancould be done with data collected through PERCS, though this comes at the cost of a reduced (though the sample size. This tradeoff demonstrations again why sequential random trials are especially well situated for MOOC experimentation will be much smaller).

\subsection{Results from PERCS}

For PERCS, we were most interested in understanding how to best sequence and space out emails with problems and emails without problems. We were not sure if users would be motivated by only problem based emails, or if, some weeks they would want no-problem based email reminders or no emails at all.  Specifically, we interested in understanding the sequential differences between the groups: 1) no emails (A), 2) no problem emails (B+C), and 3) problem emails (D+E+F+G). Each week, a user could have received one of these 3 types of emails, providing $3^3$ = 27 sequences to compare (i.e., (1,1,1), (1,1,2), (1,1,3), (1,2,1), (1,2,2), (1,2,3), ?, (3,3,2), (3,3,3)). For users in each of these sequences, we create a confidence interval for the log number of course clicks throughout the entire course. The results are in table blah

Table showing top 5 sequences and bottom 5 sequences

<Insert conclusions to be made based on table>

\section{Average treatment effects at various time points}
Instead of being interested in a sequence of interventions, researchers might want to know about the average effect of an intervention at a particular time point. To understand spaced repetition, researchers may want to know the effect of introducing review content in the 3rd week of the course? In PERCS, we wanted to know the effect of culturally personalized problem emails in weeks 2 on the subsequent week?s course activity. We also wanted to know the effect of including growth mindset framing in emails in week 3.

Sequentially randomized experiments permit the estimation of average treatment effects at various time points, where the averaging is over all prior treatments received. By re-randomizing individuals, we can separately estimate average effects at each time point and break confounding from previous time points. For example, in PERCS, if we wanted to know the average effect of culturally personalized problem emails in week 3 compared to global problem emails in week 3, we compare users receiving (all, all, F + G) to users receiving (all, all, D+E). By doing this comparison, we average over all treatments delivered prior to week 3, and isolate the effect of interest to problem emails only in week 3. 

In PERCS-AB, such a comparison is impossible. We could only compare the effects of culturally personalized problem emails for all 3 weeks, to global problem emails for all 3 weeks (F+G, F+G, F+G) vs (D+E, D+E, D+E). The effect estimated in PERCS-AB is a compounding effect of culturally problem-based and global problem-based emails instead of an average effect isolated to week 3.

In sequentially randomized trials average treatment effects can also be estimated for outcomes measured after the next re-randomization (sometimes called delayed effects).  For example, for PERCS, in addition to understanding the average effect of culturally personalized problem emails in week 2, on week 3 course activity, we are also able to understand the average effect of culturally personalized problem emails in week 2, on week 4 course activity (and other outcomes such as course completion). In this estimation, one would average over both week 1 treatment and week 3 treatment. This delayed effect cannot be estimated in PERCS-AB since, with no re-randomization after week 2, the estimate will be confounded by treatment in week 3.

\subsection{The Difference Between Average Treatment Effects and Sequence Effects}

Research questions on average treatment effects often seem similar to questions regarding sequence effects. In order to elucidate the difference, below are 3 types of questions that may be of interest to researchers:

1. What is the effect on week 3 course activity of getting any email in week 2, after not receiving an email prior? Compare (A, B+C+D+E+F+G, all) vs (A, A, all)

2. What is the average effect on week 3 course activity of getting any email in week 2, on average (averaging over all prior treatment)? Compare (all, B+C+D+E+F+G, all) vs (all, A, all)

3. What is the effect on week 3 course activity, of getting emails each week? Compare (B+C+D+E+F+G, B+C+D+E+F+G, B+C+D+E+F+G) vs (A, A, A)

Questions 1 and 3 are questions of comparing sequences of treatments, while question 2 is about average treatment effects. Note that all 3 questions can be answered by PERCS, but only questions 3 can be answered by PERCS-AB.

Also, one advantage of analyzing average treatment effects is that the sample size is typically larger than comparing sequences of treatments. The number of users used to make the comparison is much larger, since the comparison doesn?t restrict users based on what they received before or after the given week of interest.

\subsection{Results from PERCS}

In PERCS, we were interested in two average treatment effects. We wanted to know the effect on the subsequent week?s course activity of culturally personalized problem emails in weeks 1, 2, and 3. We also wanted to know the effect of including growth mindset framing in emails in weeks 1, 2, 3.

PERCS, throw in tables for JLS paper
Also say growth mindset didn?t appear to have an effect. Maybe put in table here just to show comparison.

Table 3:Log odds ratios for logistic regression model with the outcome being the binary measure of (1) the user clicks anything in the course during the week after receiving an email vs (0) the user does not click anything in the course in the subsequent week. The baseline is no email. 

\section{Personalization of interventions with Sequentially Randomized Trials}

MOOCs are notable for the high degree of diversity across their learner populationsIn MOOCs, there are a large amount of diversity between learners. In addition, as learners progress through a course, there is even diversity within a learner:; a learner?s engagement patterns may evolve from the initial weeks of a course to later weeks as their goals, knowledge, and experience changea learner?s engagement in the first week of the course can change in later weeks.   Due to this diversity, interventions may not always have the same effect. If anone intervention works for a specificone user at a givenone time, that intervention may not be effective it does not mean it will work for a different user, or even the same user, at a different time.  Personalizing treatment, by discovering when and for whom certain treatments are most effective, is critical. 

In literature, learning how to personalize treatment is synonymous with discovering moderators [cite]. Moderators are subject-specific variables which change the efficacy of anthe intervention. For example, if a MOOC intervention works better for older users than younger users, then age is a moderator and can then be used to personalize the intervention; after discovering age is a moderator, one may only deliver the intervention to older learners only. Some moderators can be discovered using A/B trials, however, sequentially randomized trials permits the discovery of two other types of moderators: additional baseline sequence moderators and mid-course moderators.

\subsection{Baseline sequence moderators}

Baseline variables are variables measured prior to the first treatment randomization and which can be treated as fixed for the period of a study. Baseline variables include learner characteristics (e.g., gender, location, age, prior courses taken) and course activity measured prior to the first randomization (e.g., whether the users has taken the course previously, scores on early assignments, survey responses at the beginning of the course). Often these variables moderate the effect of treatments and can be used for personalization. Discovering baseline moderators helps understand how to personalize interventions to account for diversity between different learners.

Sequential randomized trials and A/B tests both permit the discovery of baseline moderators. However, in sequential randomized trials, because users receiving a larger variety of sequences of interventions, this permits the discovery of baseline moderators for a larger number of intervention sequences, leading to a richer and more specific understanding of the moderating effects of various learner characteristics.

As an exampleTo exemplify, in both PERCS and PERCS-AB, one could answer the question: is the effect of 3 weeks of culturally personalized problem emails (compared to 3 weeks of non-personalized problem emails) different for lndian learners compared to US learners? However, in PERCS, one is able to evaluate the moderation of learners? location on a larger variety of treatment sequence comparisons. Indeed, the PERCS design allows an experimenter to evaluate the moderation of location on every possible sequence of interventions in the space under consideration.  One could also answer: is the effect of sequences which vary personalized and non-personalized problem emails (compared to 3 weeks of non-personalized problem emails) different for lndian learners compared to US learners? PERCS-AB is not able to answer this second question since no users are re-randomized to receive both personalized and non-personalized emails throughout the course. PERCS-AB is only able to evaluate moderation of baseline variables on the small number of sequences in the trial.

\subsection{Mid-course moderators}

Baseline moderators are important for personalizing initial treatment (or treatment sequences), however, understanding how to change treatment based on variables measured throughout the course --, i.e., mid-course moderators --, is critical. Discovering mid-course moderators tells practitioners how to personalize interventions throughout the course to account for diversity both between different users and within a user over time. 

Unlike A/B tests, sequential randomized trials permit the discovery of mid-course moderators. Statistically, due to bias introduced when including post-randomization variables in analyses, one can only discover moderator variables measured prior to randomization. By re-randomizing in sequentially randomized trials, moderators measured before each of the randomizations (which now includes mid-course data) can be discovered. 
<Should I further explain here the specifics, like I still have to preserve ordering, I can only assess there moderation on future treatment>

To exemplify, in PERCS, we hypothesized that growth mindset framing in emails sent at the end of week three only works well for students who were inactive during week 3, because they would benefit from the growth mindset encouragement. Because users were randomized again at the end of week 3, we can use PERCS data to assess how week 3 activity moderates the effect of growth mindset emails (sent at the end week 3) on week 4 activity. In PERCS-AB, week three course activity cannot be assessed as a moderator in PERCS-AB since it was measured after the one and only randomization in week one. 

We can also evaluate mid-course moderators that include previous treatment. For example, we may think that responsiveness to previous treatment could inform how to personalize future treatment. Those that were responsive should continue getting the same treatment while those that were non-responsive should get assigned different treatment. In PERCS, we hypothesized that growth mindset emails are more effective for users indicating they liked growth mindset in the previous week and users indicating they did not like non-growth mindset in the previous week. More specifically, there are four groups of learners: Group 1 are learners who received growth mindset framing in week one and had course activity in week two (i.e., growth mindset responders), Group 2 are learners who received growth mindset framing in week one and had no course activity in week two (i.e., growth mindset non-responders), Group 3 are learners who received no growth mindset framing in week one and had course activity in week two (i.e., no growth mindset responders), Group 4 are learners who received no growth mindset framing in week one and had no course activity in week two (i.e., no growth mindset non-responders). We expected growth mindset framing in week two emails to benefit Groups 1 and 4 more than Groups 2 and 3. By re-randomizing at the end of week two, we assess moderation by comparing treatment effects of growth mindset framing in week two emails for Groups 1 and 4 vs Groups 2 and 3.

Discovering how to personalize based on mid-course activity is one of the major benefits of sequential randomized trials. There are many other examples: . These discoveries allow educators to adapt content and interventions to meet the needs of learners as they dynamically transition throughout the course. Also, as learning content optimization starts to happen in real-time (i.e., reinforcement learning), knowing which real-time variables to measure and use for online optimization is critical. Sequentially randomized trials permit this discovery.

sentence like this herev but for within leaners: Discovering baseline moderators helps understand how to personalize interventions to account for diversity between different learners.

\subsection{Results from PERCS}

For PERCS, we were most interested in previous week?s course activity as a mid-course moderator. We wanted to see how different types of emails effect active and inactive users differently. Problem based emails may encourage or discourage inactive users. Not sure
Figure blah shows the results
<Insert conclusions to be made based on table>

\section{implications for practice}

This section outlines some useful considerations for researchers who are interested in designing and running sequential randomized trials for scaled learning environments. First, before thinking about trial specifics, researchers should always remember that experiments are created to inform scientific and answer questions about interventions. Deciding if a sequential randomized trial is the correct trial design depends purely upon the scientific questions of interest. For example, if researchers are not interested in understanding interventions which adapt and change throughout the course, running a sequential randomized trial is unnecessary. In PERCS, for example, if we, apriori, only cared about comparing interventions which send the same email all three weeks (because we think that what email was best in week one will be the best email in weeks two and three), then PERCS-AB would be a sufficient trial design.

If running a sequential randomized trial is best, there are also important considerations for creating the design.  All intervention sequences in a sequential randomized trial should be useful, feasible, and scalable. It is useless to evaluate intervention sequences which could never be done in practice or which are knowingly deleterious. For example, suppose a researcher was curious about optimal ordering of course content and, in turn, sequentially randomized learners to various sequences of content. If content B requires information taught in content A, none of the sequences in the experiment should place content B before content A. For another example, in PERCS, because currently there is not a completely automated way to send emails at any time, we only sent emails once a week. We did not explore the possibility of send emails many times per week (e.g., re-randomizing email sending every day) because, in practice, interventions which require manual email sending every day would not be feasible for MOOC instructors.

As in any other trial design, sample size and power calculations are important for sequentially randomized trials. Sample size calculations should be based off of the most important research questions the trial intends to answer. Since there are a larger number of possible treatment sequences in a sequentially randomized trial, calculating power and sample size requires researchers to consider which subset of users will be randomized to the sequences of interest. Once understanding which users will be used in the given comparison, sample size calculations are similar to A/B test sample size formulae for both comparing interventions and discovering moderators. 
Due to there more divisions of users to various sequences and a richer set of answerable research questions, sample sizes usually need to be larger for sequentially randomized trials (compared to A/B tests). If a researcher were only really interested in comparing two sequences of interventions and had  limited sample size, then it may be best to run an A/B test on those two sequences and forgo answers to other questions. The research may also consider changing the randomization probabilities. For example, in PERCS, if we mostly cared about comparing culturally personalized problem emails to global problem emails, we might change the weekly randomization probabilities in Table 1 to favor these two interventions.



\newpage

\section{Page 1 for figures and tables}

\newpage

\section{Page 2 for figures and tables}

\newpage

\section{Page 3 for figures and tables}

\newpage

\section{Page for references}



\newpage
\newpage
\section{Introduction}

The \textit{proceedings} are the records of a conference.\footnote{This
  is a footnote}  ACM seeks
to give these conference by-products a uniform, high-quality
appearance.  To do this, ACM has some rigid requirements for the
format of the proceedings documents: there is a specified format
(balanced double columns), a specified set of fonts (Arial or
Helvetica and Times Roman) in certain specified sizes, a specified
live area, centered on the page, specified size of margins, specified
column width and gutter size.

\section{The Body of The Paper}
Typically, the body of a paper is organized into a hierarchical
structure, with numbered or unnumbered headings for sections,
subsections, sub-subsections, and even smaller sections.  The command
\texttt{{\char'134}section} that precedes this paragraph is part of
such a hierarchy.\footnote{This is a footnote.} \LaTeX\ handles the
numbering and placement of these headings for you, when you use the
appropriate heading commands around the titles of the headings.  If
you want a sub-subsection or smaller part to be unnumbered in your
output, simply append an asterisk to the command name.  Examples of
both numbered and unnumbered headings will appear throughout the
balance of this sample document.

Because the entire article is contained in the \textbf{document}
environment, you can indicate the start of a new paragraph with a
blank line in your input file; that is why this sentence forms a
separate paragraph.

\subsection{Type Changes and {\itshape Special} Characters}

We have already seen several typeface changes in this sample.  You can
indicate italicized words or phrases in your text with the command
\texttt{{\char'134}textit}; emboldening with the command
\texttt{{\char'134}textbf} and typewriter-style (for instance, for
computer code) with \texttt{{\char'134}texttt}.  But remember, you do
not have to indicate typestyle changes when such changes are part of
the \textit{structural} elements of your article; for instance, the
heading of this subsection will be in a sans serif\footnote{Another
  footnote here.  Let's make this a rather long one to see how it
  looks.} typeface, but that is handled by the document class file.
Take care with the use of\footnote{Another footnote.}  the
curly braces in typeface changes; they mark the beginning and end of
the text that is to be in the different typeface.

You can use whatever symbols, accented characters, or non-English
characters you need anywhere in your document; you can find a complete
list of what is available in the \textit{\LaTeX\ User's Guide}
\cite{Lamport:LaTeX}.

\subsection{Math Equations}
You may want to display math equations in three distinct styles:
inline, numbered or non-numbered display.  Each of
the three are discussed in the next sections.

\subsubsection{Inline (In-text) Equations}
A formula that appears in the running text is called an
inline or in-text formula.  It is produced by the
\textbf{math} environment, which can be
invoked with the usual \texttt{{\char'134}begin\,\ldots{\char'134}end}
construction or with the short form \texttt{\$\,\ldots\$}. You
can use any of the symbols and structures,
from $\alpha$ to $\omega$, available in
\LaTeX~\cite{Lamport:LaTeX}; this section will simply show a
few examples of in-text equations in context. Notice how
this equation:
\begin{math}
  \lim_{n\rightarrow \infty}x=0
\end{math},
set here in in-line math style, looks slightly different when
set in display style.  (See next section).

\subsubsection{Display Equations}
A numbered display equation---one set off by vertical space from the
text and centered horizontally---is produced by the \textbf{equation}
environment. An unnumbered display equation is produced by the
\textbf{displaymath} environment.

Again, in either environment, you can use any of the symbols
and structures available in \LaTeX\@; this section will just
give a couple of examples of display equations in context.
First, consider the equation, shown as an inline equation above:
\begin{equation}
  \lim_{n\rightarrow \infty}x=0
\end{equation}
Notice how it is formatted somewhat differently in
the \textbf{displaymath}
environment.  Now, we'll enter an unnumbered equation:
\begin{displaymath}
  \sum_{i=0}^{\infty} x + 1
\end{displaymath}
and follow it with another numbered equation:
\begin{equation}
  \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
\end{equation}
just to demonstrate \LaTeX's able handling of numbering.

\subsection{Citations}
Citations to articles~\cite{bowman:reasoning,
clark:pct, braams:babel, herlihy:methodology},
conference proceedings~\cite{clark:pct} or maybe
books \cite{Lamport:LaTeX, salas:calculus} listed
in the Bibliography section of your
article will occur throughout the text of your article.
You should use BibTeX to automatically produce this bibliography;
you simply need to insert one of several citation commands with
a key of the item cited in the proper location in
the \texttt{.tex} file~\cite{Lamport:LaTeX}.
The key is a short reference you invent to uniquely
identify each work; in this sample document, the key is
the first author's surname and a
word from the title.  This identifying key is included
with each item in the \texttt{.bib} file for your article.

The details of the construction of the \texttt{.bib} file
are beyond the scope of this sample document, but more
information can be found in the \textit{Author's Guide},
and exhaustive details in the \textit{\LaTeX\ User's
Guide} by Lamport~\shortcite{Lamport:LaTeX}.

This article shows only the plainest form
of the citation command, using \texttt{{\char'134}cite}.

Some examples.  A paginated journal article \cite{Abril07}, an enumerated
journal article \cite{Cohen07}, a reference to an entire issue \cite{JCohen96},
a monograph (whole book) \cite{Kosiur01}, a monograph/whole book in a series (see 2a in spec. document)
\cite{Harel79}, a divisible-book such as an anthology or compilation \cite{Editor00}
followed by the same example, however we only output the series if the volume number is given
\cite{Editor00a} (so Editor00a's series should NOT be present since it has no vol. no.),
a chapter in a divisible book \cite{Spector90}, a chapter in a divisible book
in a series \cite{Douglass98}, a multi-volume work as book \cite{Knuth97},
an article in a proceedings (of a conference, symposium, workshop for example)
(paginated proceedings article) \cite{Andler79}, a proceedings article
with all possible elements \cite{Smith10}, an example of an enumerated
proceedings article \cite{VanGundy07},
an informally published work \cite{Harel78}, a doctoral dissertation \cite{Clarkson85},
a master's thesis: \cite{anisi03}, an online document / world wide web
resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03}
and \cite{Lee05} and (Case 3) a patent \cite{JoeScientist001},
work accepted for publication \cite{rous08}, 'YYYYb'-test for prolific author
\cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might contain
'duplicate' DOI and URLs (some SIAM articles) \cite{Kirschmer:2010:AEI:1958016.1958018}.
Boris / Barbara Beeton: multi-volume works as books
\cite{MR781536} and \cite{MR781537}.

A couple of citations with DOIs: \cite{2004:ITE:1009386.1010128,
  Kirschmer:2010:AEI:1958016.1958018}.

Online citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.


\subsection{Tables}
Because tables cannot be split across pages, the best
placement for them is typically the top of the page
nearest their initial cite.  To
ensure this proper ``floating'' placement of tables, use the
environment \textbf{table} to enclose the table's contents and
the table caption.  The contents of the table itself must go
in the \textbf{tabular} environment, to
be aligned properly in rows and columns, with the desired
horizontal and vertical rules.  Again, detailed instructions
on \textbf{tabular} material
are found in the \textit{\LaTeX\ User's Guide}.

Immediately following this sentence is the point at which
Table~\ref{tab:freq} is included in the input file; compare the
placement of the table here with the table in the printed
output of this document.

\begin{table}
  \caption{Frequency of Special Characters}
  \label{tab:freq}
  \begin{tabular}{ccl}
    \toprule
    Non-English or Math&Frequency&Comments\\
    \midrule
    \O & 1 in 1,000& For Swedish names\\
    $\pi$ & 1 in 5& Common in math\\
    \$ & 4 in 5 & Used in business\\
    $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{table}

To set a wider table, which takes up the whole width of the page's
live area, use the environment \textbf{table*} to enclose the table's
contents and the table caption.  As with a single-column table, this
wide table will ``float'' to a location deemed more desirable.
Immediately following this sentence is the point at which
Table~\ref{tab:commands} is included in the input file; again, it is
instructive to compare the placement of the table here with the table
in the printed output of this document.


\begin{table*}
  \caption{Some Typical Commands}
  \label{tab:commands}
  \begin{tabular}{ccl}
    \toprule
    Command &A Number & Comments\\
    \midrule
    \texttt{{\char'134}author} & 100& Author \\
    \texttt{{\char'134}table}& 300 & For tables\\
    \texttt{{\char'134}table*}& 400& For wider tables\\
    \bottomrule
  \end{tabular}
\end{table*}
% end the environment with {table*}, NOTE not {table}!

It is strongly recommended to use the package booktabs~\cite{Fear05}
and follow its main principles of typography with respect to tables:
\begin{enumerate}
\item Never, ever use vertical rules.
\item Never use double rules.
\end{enumerate}
It is also a good idea not to overuse horizontal rules.


\subsection{Figures}

Like tables, figures cannot be split across pages; the best placement
for them is typically the top or the bottom of the page nearest their
initial cite.  To ensure this proper ``floating'' placement of
figures, use the environment \textbf{figure} to enclose the figure and
its caption.

This sample document contains examples of \texttt{.eps} files to be
displayable with \LaTeX.  If you work with pdf\LaTeX, use files in the
\texttt{.pdf} format.  Note that most modern \TeX\ systems will convert
\texttt{.eps} to \texttt{.pdf} for you on the fly.  More details on
each of these are found in the \textit{Author's Guide}.

\begin{figure}
\includegraphics{fly}
\caption{A sample black and white graphic.}
\end{figure}

\begin{figure}
\includegraphics[height=1in, width=1in]{fly}
\caption{A sample black and white graphic
that has been resized with the \texttt{includegraphics} command.}
\end{figure}


As was the case with tables, you may want a figure that spans two
columns.  To do this, and still to ensure proper ``floating''
placement of tables, use the environment \textbf{figure*} to enclose
the figure and its caption.  And don't forget to end the environment
with \textbf{figure*}, not \textbf{figure}!

\begin{figure*}
\includegraphics{flies}
\caption{A sample black and white graphic
that needs to span two columns of text.}
\end{figure*}


\begin{figure}
\includegraphics[height=1in, width=1in]{rosette}
\caption{A sample black and white graphic that has
been resized with the \texttt{includegraphics} command.}
\end{figure}

\subsection{Theorem-like Constructs}

Other common constructs that may occur in your article are the forms
for logical constructs like theorems, axioms, corollaries and proofs.
ACM uses two types of these constructs:  theorem-like and
definition-like.

Here is a theorem:
\begin{theorem}
  Let $f$ be continuous on $[a,b]$.  If $G$ is
  an antiderivative for $f$ on $[a,b]$, then
  \begin{displaymath}
    \int^b_af(t)\,dt = G(b) - G(a).
  \end{displaymath}
\end{theorem}

Here is a definition:
\begin{definition}
  If $z$ is irrational, then by $e^z$ we mean the
  unique number that has
  logarithm $z$:
  \begin{displaymath}
    \log e^z = z.
  \end{displaymath}
\end{definition}

The pre-defined theorem-like constructs are \textbf{theorem},
\textbf{conjecture}, \textbf{proposition}, \textbf{lemma} and
\textbf{corollary}.  The pre-defined de\-fi\-ni\-ti\-on-like constructs are
\textbf{example} and \textbf{definition}.  You can add your own
constructs using the \textsl{amsthm} interface~\cite{Amsthm15}.  The
styles used in the \verb|\theoremstyle| command are \textbf{acmplain}
and \textbf{acmdefinition}.

Another construct is \textbf{proof}, for example,

\begin{proof}
  Suppose on the contrary there exists a real number $L$ such that
  \begin{displaymath}
    \lim_{x\rightarrow\infty} \frac{f(x)}{g(x)} = L.
  \end{displaymath}
  Then
  \begin{displaymath}
    l=\lim_{x\rightarrow c} f(x)
    = \lim_{x\rightarrow c}
    \left[ g{x} \cdot \frac{f(x)}{g(x)} \right ]
    = \lim_{x\rightarrow c} g(x) \cdot \lim_{x\rightarrow c}
    \frac{f(x)}{g(x)} = 0\cdot L = 0,
  \end{displaymath}
  which contradicts our assumption that $l\neq 0$.
\end{proof}

\section{Conclusions}
This paragraph will end the body of this sample document.
Remember that you might still have Acknowledgments or
Appendices; brief samples of these
follow.  There is still the Bibliography to deal with; and
we will make a disclaimer about that here: with the exception
of the reference to the \LaTeX\ book, the citations in
this paper are to articles which have nothing to
do with the present subject and are used as
examples only.
%\end{document}  % This is where a 'short' article might terminate



\appendix
%Appendix A
\section{Headings in Appendices}
The rules about hierarchical headings discussed above for
the body of the article are different in the appendices.
In the \textbf{appendix} environment, the command
\textbf{section} is used to
indicate the start of each Appendix, with alphabetic order
designation (i.e., the first is A, the second B, etc.) and
a title (if you include one).  So, if you need
hierarchical structure
\textit{within} an Appendix, start with \textbf{subsection} as the
highest level. Here is an outline of the body of this
document in Appendix-appropriate form:
\subsection{Introduction}
\subsection{The Body of the Paper}
\subsubsection{Type Changes and  Special Characters}
\subsubsection{Math Equations}
\paragraph{Inline (In-text) Equations}
\paragraph{Display Equations}
\subsubsection{Citations}
\subsubsection{Tables}
\subsubsection{Figures}
\subsubsection{Theorem-like Constructs}
\subsubsection*{A Caveat for the \TeX\ Expert}
\subsection{Conclusions}
\subsection{References}
Generated by bibtex from your \texttt{.bib} file.  Run latex,
then bibtex, then latex twice (to resolve references)
to create the \texttt{.bbl} file.  Insert that \texttt{.bbl}
file into the \texttt{.tex} source file and comment out
the command \texttt{{\char'134}thebibliography}.
% This next section command marks the start of
% Appendix B, and does not continue the present hierarchy
\section{More Help for the Hardy}

Of course, reading the source code is always useful.  The file
\path{acmart.pdf} contains both the user guide and the commented
code.

\begin{acks}
  The authors would like to thank Dr. Yuhua Li for providing the
  MATLAB code of the \textit{BEPS} method.

  The authors would also like to thank the anonymous referees for
  their valuable comments and helpful suggestions. The work is
  supported by the \grantsponsor{GS501100001809}{National Natural
    Science Foundation of
    China}{http://dx.doi.org/10.13039/501100001809} under Grant
  No.:~\grantnum{GS501100001809}{61273304}
  and~\grantnum[http://www.nnsf.cn/youngscientists]{GS501100001809}{Young
    Scientists' Support Program}.

\end{acks}

==> old_main_body.tex <==
\section{Introduction}\label{sec:introduction}

In order to continually improve learner experience and maintain engagement, scaled digital learning environments (SDLEs), such as Massively Open Online Courses (MOOCs), intelligent tutoring systems, and open-ended digital educational games, utilize \textit{interventions}. Interventions are modifications made to the learning environment or learners' experience of it, including changing current course content, prompting users to return to the course, or providing additional learning resources (e.g.,\cite{Davis_2018}). It is common to find interventions which are technological, pedagogical, or programmatic in their implementation.

In SDLEs, there is typically diversity both \textit{between} learners (e.g., different learners have different needs) \cite{Kizilcec_2017}, and \textit{within} a learner over time (e.g., a learner's engagement may change throughout a course) \cite{Kizilcec_2013}. To accommodate this diversity, interventions should be adaptive. \textit{Adaptive interventions} can change based on the type of learner (to account for diversity between learners) and change as a learner progresses through the course (to account for diversity within a learner) \cite{almirall_2018}. For example, consider an intervention which introduces review problems throughout a course. The frequency of review problems might adapt based on the week (e.g., learners may not need to review as often in later weeks). The frequency of review might also adapt based on the learner's performance (e.g., building upon work on theories of \emph{spaced repetition} \cite{reynolds1964effects}).

Due to the large number of users and ease of content manipulation in SDLEs, randomized controlled trials (e.g., A/B tests) are often used to evaluate education intervention options (e.g., learning activity). Typically, these experiments are single-randomized trials where each subject is randomized once, and assigned to a single intervention option for the entire trial. However, when the goal is to design a high-quality adaptive intervention in SDLEs, researchers may have important questions about the sequencing, timing, and personalization of intervention options which cannot be answered by A/B tests.  

In this work, we discuss and demonstrate the advantages of an experimental design for developing high-quality adaptive interventions in SDLEs: the \textit{sequential randomized trial} (SRT). In SRTs, a subject is randomized several times to different intervention options throughout the experiment. Sequential randomization is beneficial over one-time randomization for several reasons.  Firstly, by re-randomizing, subjects receive a variety of intervention sequences, and these various sequences can be compared to discover the optimal intervention sequence.  Secondly, instead of only being able to assess the overall effect of getting one particular treatment, sequential randomization lets researchers discover effects at smaller time-scales (e.g., treatment A does better in week 2 of the course, but treatment B does better in week 3 of the course). These discoveries inform at what time points certain interventions are most effective. Thirdly, re-randomization permits the discovery of important variables measured throughout the course for adapting and personalizing an intervention. As opposed to only being able to discover baseline personalization variables (e.g., treatment A works better for women), we can also discover mid-course personalization variables (treatment A works better for subjects with who have been active in the course during the previous day).
 
%SRTs are particularly advantageous when aiming to develop an adaptive intervention in SDLEs. First, SRTs inform how to adapt interventions to meet the needs of all learners at all times within the diverse learner population of an SDLE. Second, the fully computer-mediated nature of many SDLEs means that there are typically a large number of possible modifications and intervention options. SRTs can maximally leverage the large sample sizes of SRTs, sometimes on the order of tens of thousands of learners \cite{Kizilcec_2017}, by comparing, with power, a larger variety of treatment sequences than an A/B test. For example, course designers can modify the ordering of course content, as well as layout, appearance (color, texture), arrangement, and default settings of interfaces. Third, SRTs are beneficial for research in SDLEs from a practical perspective. In clinical or classroom settings, reassignment of intervention options adds a layer of complexity, making intervention delivery difficult. In SDLEs, where interventions can be delivered quickly and at scale, the burden of re-randomization and delivering a variety of intervention options is minimized. SRTs leverage this lower cost of re-randomization within a trial by repeatedly re-assigning users to new treatments.  

%SRTs are particularly useful as exploratory trials (as opposed to confirmatory), to help researchers narrow down intervention options and discover the best (which can then be further validated). SDLEs are also better able to implement a personalized adaptive intervention based on results of a SRT. In face-to-face or blended learning environments it is often impractical to deliver personalized interventions to each student, as the nature of the face-to-face experience tends to preclude individual-level learning from the instructor. 

The paper is structured as follows. First, we provide an overview of related prior work on experimentation and personalized interventions in SDLEs in Section \ref{sec:prior-work}. In Section \ref{sec:seqential-randomization}, we formally introduce SRTs and compare them to other common trial designs.
 In Section \ref{sec:srt_examples}, to motivate the design we describe a novel
 %\footnote{The authors are not aware of any previous SRT designs being used in MOOC research to date.}
 SRT performed in MOOCs, the Problem-based Email Reminder Coursera Study (PERCS). 
 This was an experiment aiming to
 improve student retention in an online course by developing a high-quality adaptive email intervention which 
 leverages aspects of cultural diversity and inclusion \cite{Aceves_2014a}. This case study both serves to illustrate the advantages of SRTs and provide context regarding implementation and analysis. Section \ref{seq_time_pers} details three specific advantages of running SRTs. These advantages are exemplified by showing specific results from PERCS. We conclude by providing some practical recommendations for researchers designing their own SRTs in Section \ref{sec:implications-for-practice}.

\section{Prior Work}\label{sec:prior-work}

\subsection{Adaptive Interventions}

Adaptive interventions have been shown to be useful in SDLEs, and have been used extensively in web-based adaptive educational systems \cite{Brusilovsky_2003}. For instance, in \cite{Pardos_2017} learners were provided personalized content recommendations based on their clickstream data, and in \cite{Davis_2018b}, learners were provided personalized feedback on their learning plans. Adaptive sequences of interventions have also been developed in MOOCs, and \cite{David_2016} used adaptive sequencing for problems based on predictions of student knowledge acquisition. Similarly \cite{Davis_2018} chose quiz questions based on course content accessed previously by the learner. While these are only a few examples of adaptive interventions in large scale learning environments, they motivate our desire to improve the process by which such interventions are developed. 


In the work discussed, adaptive interventions were developed using learning theory and intention \cite{Davis_2018}, or prediction and machine learning \cite{Pardos_2017, Yu_2017, David_2016}.  In all examples, experimentation was not used to develop the adaptive intervention. In some cases \cite{Davis_2018, David_2016}, experimentation was used for evaluating the adaptive intervention. In these cases, an A/B test is used to compare the designed intervention to a control.
%In contrast, the overarching aim in SRTs is to use experimentation to decide how to best personalize and adapt an intervention. 

%SRTs do not optimize throughout the trial and can be thought of as pure exploration. See Section~\ref{sec:compare} for more details on these differences.

Reinforcement learning techniques, such as multi-armed bandits and contextual bandits, are a type of adaptive interventions which combine exploration (often done through implicit experimentation) and optimization. They use real-time data to learn how to adapt and have also been shown to be useful in SDLEs \cite{Liu_2014b, Clement_2013, Segal_2018, Rafferty_2018}.

\subsection{Experimental Designs}

Experimentation in SDLEs is a common tool for evaluating interventions. 
Unlike quasi- or natural experimental settings \citep[e.g.,][]{gonzalez_2015, Mullaney_2015}, by randomly assigning interventions, effects of interventions can be separated from effects of confounders (variables that relate both to the type of treatment received and to subsequent outcomes).

A/B tests are a valuable experimental design for improving content and evaluating interventions in MOOCs \cite{savi_2017}. In \cite{Renz_2016}, for example, A/B tests evaluated emails and course on-boarding to improve learner engagement and prevent dropout. In \cite{Davis_2016}, A/B tests were used to test the effectiveness of self-regulated learning strategies. Kizilcec and Brooks \cite{Kizilcec_2017} survey prior work utilizing A/B tests in MOOCs to evaluate nudge interventions and test theory-driven course content changes.


There has also been considerable work in other types of experimental designs beyond A/B testing in SDLEs. \textit{Factorial designs}  \citep[e.g.,][]{Lomas_2013} are common ways to evaluate multiple experimental factors simultaneously. 
%Factorial designs are still single-randomized trials, however, factorial designs can be incorporated into SRTs, as we demonstrate in the design of PERCS in Section \ref{sec:percs}. 
\textit{Automatic experimentation} \citep[e.g.,][]{Liu_2014}, where algorithms are used to search through different intervention options, is another alternative to A/B testing. Though automatic exploration of intervention options may be more efficient, intervention options are still evaluated with single-randomized trials. \textit{Adaptive experimental designs} change the randomization probabilities to favor efficacious treatment. With the goal of both evaluating treatment and helping learners currently in the trial \cite{Chow_2008}. Adaptive designs have been used in SDLEs \cite{Williams_2018}. We address the differences between SRTs and these other kinds of designs in Section \ref{sec:compare}.


\section{Sequential Randomized Trials} \label{sec:seqential-randomization}
\subsection{An Overview}

SRTs are trials where an individual is randomized multiple times throughout the course of the trial. Suppose there are two intervention options, such as learners receiving videos taught by a female instructor (intervention A) or a male instructor (intervention B). The simplest example of a SRT would be: During week 1, users have a 50\% chance of receiving intervention A and a 50\% chance of receiving intervention B.  During week 2, users are re-randomized to another treatment. They again have a 50\% chance of receiving either intervention A or B, independent of their week 1 treatment or activity. Hence, about 25\% of users will have received one of each sequence (A, A), (A,B), (B,A), or (B,B), where the parenthetical notation means (week 1 treatment, week 2 treatment).

This simple SRT can be modified for both practical and scientific reasons. Common modifications include using different time durations (e.g., re-randomize every month), increasing the number of time points (e.g., each person is randomized 10 times instead of twice), changing the number of treatments (e.g., A vs B vs C instead of A vs B, or A vs B in week 1 and C vs D in week 2), and altering the randomization scheme (e.g., not having uniform randomization probabilities each week, or, in week 2, only re-randomizing inactive users).

Trials with sequential randomization \cite{Lavori_2004, Lavori_2000} have become relatively common in clinical settings \cite{Lei_2011} and are becoming more prevalent in educational settings \cite{almirall_2018}.  Two of the most common types of SRTs are Sequential Multiple Assignment Randomized Trials (SMARTs) \cite{Murphy_2005}, and Micro-randomized Trials (MRTs) \cite{Klasnja_2015}. In a prototypical SMART, individuals are first randomized to one of two different treatment options. Then, at a pre-specified decision point following initial intervention,  users who did not respond to initial treatment are re-randomized, while users who did respond to initial treatment are not re-randomized and continue with the efficacious initial treatment \cite{Pelham_2016}. MRTs have been mostly used in the mobile health space, where interventions (such as delivering reminders on a subject's phone) can be delivered quickly and frequently. Due to the high frequency of delivery, users in an MRT are typically re-randomized hundreds or thousands of times to identify when interventions should be delivered to maximize short-term impact.


\subsection{Comparisons to Other Designs}\label{sec:compare}

\subsubsection{A/B Testing}

SRTs are distinctive from many other types of common trial designs. In A/B tests (often called a 2-arm randomized controlled trial in healthcare and education), each subject is randomized \textbf{one time} to either intervention A or intervention B. SRTs randomize subjects several times, causing them to receive multiple treatments throughout the trial. Through sequential randomization, researchers can answer many more questions about sequencing, timing, and personalizing adaptive interventions, as described in Section~\ref{seq_time_pers}.

A/B tests can still be used to evaluate adaptive interventions. For example, if treatment A is defined as an adaptive intervention (e.g., a fixed sequence of different intervention options) and treatment B is defined as a control, an A/B test can compare the adaptive intervention to the control with a single randomization. Unfortunately, since randomization only occurs once, this trial is limited in answering questions about sequencing, timing, and personalizing.

A/B tests are often used in confirmatory trials. Confirmatory trials are trials used to ensure strong evidence (or additional evidence) of a treatment's efficacy, where one intervention is the treatment of interest and the other intervention is the control. Confirmatory trials differ from exploratory trials, which are typically done in the early stages of intervention development to help researchers narrow down intervention options, understand efficacious intervention components, and learn how individuals' characteristics change intervention efficacy. SRTs are specifically useful as an exploratory trial in SDLEs, with the goal being to leverage the large population of learners to explore a large number of possible treatment sequences, and learn how to adapt those sequences. After running a SRT and developing a high quality adaptive intervention, the designed intervention sequence can be confirmed in a simple A/B confirmatory trial where the proposed intervention sequence is compared to a control \cite{Collins_2007}.


\subsubsection{Online Optimization Designs}

There are other designs (both experimental and not) which aim to optimize intervention delivery while simultaneously collecting data. In adaptive trial designs \cite{Chow_2008}, randomization probabilities are changed throughout the trial in order to both provide efficacious treatment to users, and still obtain good estimates of treatment effects. 
Online reinforcement learning methods (such as multi-armed bandit and contextual bandit algorithms) can also be used for optimizing intervention delivery \cite{Liu_2014b, Clement_2013, Segal_2018, Rafferty_2018}. These online treatment optimization techniques can provide better treatment for new subjects (based on data from previous subjects) \cite{Williams_2018}, and can also provide better treatment for the same subject at a later time (based on the subject's earlier data) \cite{Clement_2013}.

SRTs are distinctive from adaptive trial designs and online reinforcement learning methods since they do not perform any online optimization. That is, SRTs do not use data collected throughout the trial to change randomization schemes. The randomization scheme is pre-specified and stationary. In reinforcement learning language, SRTs can be seen as pure exploration with no exploitation.

Even though a SRT is not explicitly aimed to benefit learners during the trial, there are advantages of not using earlier trial data to inform future treatment allocation:
\begin{enumerate}
\item Using online optimization techniques can cause bias in estimating treatment effects \cite{Nie_2017, Rafferty_2018}. Since data collected during the trial does not change a SRT's randomization scheme, issues of bias do not arise.

\item Many reinforcement learning methods require assumptions for good performance. In multi-armed bandits \cite{Liu_2014b, Clement_2013, Rafferty_2018} and contextual bandits \cite{Lan_2016}, for example, it is assumed that prior treatment does not change the efficacy of future treatment. This assumption may not be realistic. Since SRTs do not optimize, they do not require any assumptions about the data. Instead, they provide a rich data set useful for checking such assumptions and validating the eventual use of reinforcement learning methods.

\item SRTs provide rich exploratory data for discovering which variables are valuable for informing treatment decisions, making them useful when these variables are not known (see Section \ref{sec:personalization-with-srts}). In contrast, many reinforcement learning algorithms, such as contextual bandits \cite{Lan_2016}, require the context (i.e., learner characteristics informing treatment decisions) to be specified. 

\item SRTs can actually utilize reinforcement learning methods. Batch off-policy reinforcement learning algorithms (such as Q-learning) can be applied to SRT data to discover an optimal adaptive intervention, as in \cite{Zhao_2009}.
     
\end{enumerate}


%% old phrasing that's not right
%SRTs are different from adaptive trial designs. Data from a SRT informs the development interventions which are adaptive (i.e., interventions which change throughout the course for a given user), however, the trial itself is non-adaptive. Unlike adaptive trial designs, in SRTs all users are randomized the exact same way; the randomization of new users does not change based on data collected during the trial.

%Both trial designs are advantageous, but for different reasons. If research questions are about how to personalize, adapt, and sequence a series of interventions for an individual, SRTs should be used.  If a researcher's goal is to evaluate an intervention while also hoping to improve learning outcome for users currently in the trial, then they should use adaptive designs.
%There is some work on how adaptive designs can inform how to personalize interventions (using contextual bandit algorithms)[cite], however, personalization capabilities is limited compared to SRTs (see section blah).

%They are instead used to develop interventions which adapt.  
% and they adapt within a person.

\section{Applications of SRTs} \label{sec:srt_examples}


SRTs can inform a large variety of interventions including course content sequencing, course material manipulations, and learner nudges (such as encouraging messages and problem feedback). We highlight three examples. The first two examples are hypothetical scenarios to demonstrate different types of possible SRTs. The third example, PERCS, is a SRT run in a data science MOOC and is the main working example. 

\subsection{Video Optimization} For each video in an MOOC, there are two versions, one video which shows only slides and one which shows the instructor's head occasionally interspersed with the slides \cite{Guo_2014}. Researchers are unsure about which sequence of videos are better. 
Learners might prefer only slides, some might prefer those with instructors, or some might prefer a variety of videos. Also, there may be learner characteristics that affect learner preference. For example, learners who initially performed poorly after watching an instructor video might be better off seeing a slide-only video. To provide insight into these questions and hypotheses, a researcher could run a SRT: When a learner enters a course, they are randomized initially to receive an instructor video or a slide only video. Then, after watching the first video, they are re-randomized to either instructor or slide video for the next video they watch. This continues through the entire course.

\subsection{Content Spacing} Researchers are often unsure about optimal review problem sequencing to maximize knowledge retention while minimizing review time \cite{reynolds1964effects}.  Learners may benefit from frequent review at the beginning then less frequent review later. Secondly, how should learner characteristics inform review problem spacing? Should learners who are performing well receive different problem spacing sequences than poor performing learners?
A SRT can answer these questions: For a problem recommendation system, a learner starts the recommender for a time window (e.g., 50 problems). Then, after this time period, every learner is randomized to one of 3 groups: no review, minimal review, large review. The grouping determines how often they receive previously-seen problems (for review) during the next 20 problems. If a learner is in the no review, minimal review, or large review group they will receive previously-seen problems 0\%, 5\%, or 20\% of the time, respectively. After completing the next 20 problems, each user will be re-randomized to one of the 3 groups. This randomization scheme continues. Every 20 problems completed, a user is re-randomized to one of the 3 groups.

\subsection{Problem-based Email Reminder Study (PERCS)}\label{sec:percs}


\subsubsection{Motivation}
\label{sec:rqs}

A well-known challenge in MOOCs are the low completion rates. While there are many factors contributing to MOOC dropout \cite{Greene_2015}, the goal of PERCS is to determine whether dropout can be ameliorated by using weekly email reminders to motivate learners to engage with course content. Our context of inquiry was the [redacted for review] data science MOOC, taught by one of the authors. Weekly emails were sent to learners and may have contained one or more of several factors intending to impact learner engagement (see Table~\ref{tab:probs}):
\begin{enumerate}
    \item The email could have contained a motivating data science problem to challenge the user to learn the upcoming week's content. This factor was based on evidence from the problem-based learning literature suggesting that situating instruction in the context of problems is an effective way to engage learners \cite{barrows1985design}.
    \item  The email might also have contained a location specific primer and a data science problem relevant to that user's specific culture (e.g., an Indian user might receive a problem about Bollywood or weather patterns in India). This factor was based on the work in the culturally relevant and culturally responsive pedagogy communities, where situating instruction in a manner that considers the local context is seen as beneficial \cite{Aceves_2014a}.
    \item The email may have utilized growth mindset framing \cite{Dweck_2008}, a psychological framing method used to support learning. While growth mindset has been heavily studied, its effects are in dispute \cite{Kaijanaho_2018}, and growth mindset framing has seen only limited application in scaled online learning environments.
\end{enumerate}

Given these weekly email options, we hope to develop an adaptive intervention of weekly email reminders to increase engagement and reduce dropout. A high quality adaptive intervention should sequence emails in a way that promotes engagement continually through the course.  Since different emails may be more or less effective during different weeks in the course, each week, the intervention should send the most effective email for that week. Finally, since we might not expect the same email to work well for everyone, the intervention should also adapt to the learner's current course behavior. In order to develop a high quality adaptive intervention of emails, we need to answer the following research questions: 


\begin{enumerate}[label=RQ\arabic*]
    \item \textbf{Sequencing}: Which sequence of emails most improves course activity in later weeks?\label{rq1}
    \item \textbf{Timing}: Which email problem type is most effective, on average, for bringing learners back to the course during each week? \label{rq2}
    \item \textbf{Personalization}: Are certain data science problem emails more or less effective for active learners? \label{rq3}
\end{enumerate}
            
\subsubsection{Design}

\begin{figure}
    \centering
    \includegraphics[width= 0.7 \columnwidth]{img/email_structure_narrow_redacted.pdf}
    \caption{Example email structure using content which is populated based on their assigned treatments. (A) Identity activation prompt. (B) Culturally-relevant problem using data related to geographic identity. (C) Reminder to return to course. (D) Link to code for problem-based practice. (E) Growth mindset framing. (F) Link to problem solution. Elements of the same email type are grouped by color (see key).
    Learner, instructor, and course name redacted for review.}
    \label{fig:example-email}
\end{figure}

A sequentially randomized factorial trial design was an effective method to jointly address the main research questions of PERCS. At the end of weeks one, two, and three of the four-week long MOOC, learners were randomly assigned to receive one of four different email categories: an email message with a problem that reflects their geo-cultural situation based on IP address (\emph{cultural problem email}); an email with a generic, non-culture specific problem (\emph{global problem email}); an email with \emph{no problem}; or \emph{no email} at all. Those who received an email were uniformly randomly assigned to have the email be framed with or without growth mindset. 

The growth mindset factor crossed with the three email categories makes each week of PERCS a $2 \times 3$ factorial design with an additional control condition of no email. See Table~\ref{tab:probs} for each week's factorial design and randomization probabilities.


\begin{figure*}
    \centering
    \includegraphics[width = 0.8 \textwidth]{img/perts_design_trimmed.pdf}
    \caption{PERCS trial design. ``R'' indicates stages where randomization is conducted according to the probabilities in Table \ref{tab:probs}.}
    \label{fig:percs_design}
\end{figure*}

\begin{table*}[]
\begin{tabular}{ll|
>{\columncolor[HTML]{EFEFEF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |}
\cline{1-1} \cline{3-6}
\multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}No Email E_0} &  & Email E_1               & \cellcolor[HTML]{EFEFEF}No Problem Email (P_0) & \cellcolor[HTML]{EFEFEF}Global Problem Email (P_1) & \cellcolor[HTML]{EFEFEF}Cultural Problem Email (P_2) \\ \cline{1-1} \cline{3-6} 
\multicolumn{1}{|l|}{\cellcolor[HTML]{FFFFFF}0.14 (T_1)}   &  & No-Growth Mindset (G_0) & 0.14 (T_2)                                     & 0.14 (T_3)                                         & 0.14 (T_4)                                             \\ \cline{1-1} \cline{3-6} 
                                                           &  & Growth Mindset (G_1)    & 0.14 (T_5)                                     & 0.14 (T_6)                                         & 0.14 (T_7)                                             \\ \cline{3-6} 
\end{tabular}
\caption{An overview of the probability learners will be assigned to a treatment $T_n$. Individual treatments are shown in white cells, while groups of treatments are referred to by the tab row or column headers (e.g., all cultural problem emails as $P_2$)}
\label{tab:probs}
\end{table*}


Figure \ref{fig:example-email} illustrates an example email. The emails were developed in a ``cut and paste format'': When adding in a condition to an email (e.g., growth mindset framing or adding a problem), we do not change other aspects of the email, and simply insert text from the relevant condition into a consistent email template. Using the cut and paste across different conditions allowed us to attribute treatment effects purely to the condition being added, and not other aspects of the email. Emails are delivered directly using the Coursera platform's email capabilities for instructors.
 
The most novel aspect of PERCS is the sequential randomization. That is, a particular learner does not get randomized to a single email condition and remain in that treatment condition for all three weeks. Instead, as shown in Figure \ref{fig:percs_design}, each week, a learner is re-assigned (with the same randomization probabilities) to a different email condition. The randomizations across weeks are independent, hence in PERCS, there are $7^3$ ($343$) possible different email sequences students may receive.

\subsubsection{Notation}

Throughout the rest of the paper, we will be referring to specific treatments, groups of treatments, and sequences of treatments in PERCS. We introduce notation to ease our description. As shown in Table \ref{tab:probs}, $T_1, T_2, \dots, T_7$ refers to a particular email. For example, $T_2$ is an email containing no problem, and growth mindset framing. To refer to groups of emails, we used labeling contained in the column and row headers in Table \ref{tab:probs}. $E$ is used to group together conditions where any email was sent ($E_1$) vs no email being sent ($E_0$). So users in $E_1$ refer to any user receiving emails $T_2$ through $T_7$. $G$ is used to group together growth mindset emails ($G_1$) and non-growth mindset emails ($G_0$). Users in $G_0$ refer to any user receiving emails $T_5, T_6, $ or $ T_7$. $P$ is used to group together no problem emails ($P_0$), global problem emails ($P_1$), and cultural problem emails ($P_2$). Thus users in $P_1$ are are any users receiving emails $T_3$ or $T_6$.  Lastly, we use parenthetical notation to describe the sequences of emails over the three weeks, i.e., (week one treatment, week two treatment, week three treatment). As an example, we would refer to users who received a global problem email in week 1, any email in week two, and a no-growth mindset email in week three we use ($P_1, E_1, G_0$).


\subsubsection{Experimental Population}

We focused our trial on the two largest populations of learners enrolled in the course as determined by IP-address, Indian and US-based learners. All Indian and US learners who signed up for the [redacted for review] between the times of April 1, 2018 to June 10, 2018 participated in PERCS. A total of 8,681 unique learners (3,455 Indian, 5,226 US) were sent 22,073 emails. 
%% india 7717 3455
%% us 12,356 5,226

\subsubsection{A/B Testing Version of PERCS}

To highlight the advantages of sequential randomization, PERCS will be compared to the single-randomized, A/B testing version of PERCS (PERCS-AB). PERCS-AB has the exact same randomization probabilities as PERCS, however in PERCS-AB, prior to the start of week two, learners are randomized to one of the 7 email types, and are sent that exact same email type for the subsequent 3 weeks. Hence, there are only 7 possible sequences ($T_1, T_1, T_1)$, $(T_2,T_2,T_2)$, $\dots$,  $(T_7,T_7,T_7)$.


\section{Sequencing, Timing, and Personalizing Interventions through SRTs} \label{seq_time_pers}.
%or developing high quality adaptive interventiosn wtih srts

Next we highlight how SRTs can provide answers to questions regarding sequencing, timing, and personalizing interventions. For each type of question, we provide (1) an overview of the question and contextualize it within PERCS, (2) evidence of why SRTs are beneficial for answering that question as illustrated through comparing PERCS and PERCS-AB, (3) further discussion, and (4) answers to the question in the context of PERCS.

\subsection{Sequencing} \label{sec:optimal-sequence}

\subsubsection{Overview} 
When many different intervention options can be delivered at different times, proper sequencing of interventions is critical. An intervention that worked at one time, may not work at a later time. Also, receiving the same intervention multiple times may be less effective than receiving a variety of interventions. Researchers may not know which sequence of intervention options will lead to the best outcomes for learners. For PERCS, \ref{rq1} from Section~\ref{sec:rqs} refers to sequencing-- are there sequences of emails which improve course activity in the later weeks?

%\subsubsection{Research Questions}

%Research questions regarding effects of different treatment sequences include:

%For the \emph{Video Optimization} scenario we are interested in knowing throughout a course, whether learners prefer only videos with slides, only videos with instructors, or a variety. For the \emph{Content Spacing} scenario, we are interested in understanding whether learners will benefit from frequent review problems in either earlier or later time frames. Finally, for the \emph{PERCS} scenario we are interested in \ref{rq1} from Section~\ref{sec:rqs}, whether there are sequences of emails which improve course activity in the later weeks.

\subsubsection{Advantages of SRTs}

SRTs provide data that allows experimenters to compare different sequences of interventions. By re-randomizing learners, learners receive a variety of treatment sequences. In PERCS, for example, with the large sample size, there are learners who have the sequence $(T_1, T_1, T_1)$, $(T_1, T_1, T_2)$, $(T_1, T_2, T_2)$, or $(T_2, T_1, T_2)$. For the $7^3$ possible sequences of treatments, there are learners randomly assigned to each of those sequences.

By having learners randomized to all of these different sequences, researchers are now able to compare different sequences of treatment. For example, researchers could compare the effects on course activity of not receiving an email followed by two specific problem-based emails $(E_0, T_2, T_7)$ vs two different problem-based emails followed by not receiving an email ($T_3, T_4, E_0)$, by simply comparing the course activity of users randomized to these two sequences.

In A/B tests, since learners do not get re-randomized, sequence comparison can only be done for sequences where each learner received the same treatment the entire time. In PERCS-AB, learners are only randomized to 7 possible sequences and thus comparisons can only be done between these 7 sequences. If there was any benefit to receiving different interventions (and/or in a different order) then this could not be discovered by PERCS-AB. However one would note that all of the comparisons of PERCS-AB can be done with data collected through PERCS, coming at the cost of a reduced sample size. This tradeoff demonstrates again why SRTs are especially well situated for MOOC experimentation, where there is a large number of diverse participants (and thus a broad exploration might be suitable).
 
\subsubsection{Discussion}
%Comparing sequences of treatment groups

Often times, researchers are not interested in such specific sequence comparisons. Instead, they are interested in questions about sequences of groups of interventions. In this case, one could perform similar comparisons, but combining users over all of these groups. For example, in PERCS,
we can assess how often reminder emails should be sent. Is it better to space emails out weekly or bi-weekly?
%\footnote{Due to space limitations we do not describe the results here, and focus only on sharing the main RQs described in Section \ref{sec:rqs}. SRTs provide significant opportunity for broad experimental inquiry!}
To answer this question, we could compare course activity of users receiving the sequence which spaces emails out by 2-weeks $(E_1, E_0, E_1)$, to the sequence which sends emails every week $(E_1, E_1, E_1)$. The sample size for this comparison will be much larger than for the single sequence comparisons.

In addition to comparing groups of sequences, researchers might only be interested in comparing sequences for a small number of time points. For example, we could use data collected in PERCS to understand if the effects of week two problem-based emails on course activity were different based on what type of problem-based email the user had received in week one. Specifically, does getting no email vs cultural problem-based email in week one change the benefits of receiving a cultural problem email in week two?  To answer this question, we compare course activity in week two of users receiving sequences $(E_0, P_2, $any) vs ($P_2, P_2, $any). Notice we are not concerned with anything occurring in week three, so we include sequences with any treatment in week three (i.e., any includes $T_1, T_2, \dots, T_7$)

%In PERCS-AB, learners are only randomized to 7 possible sequences $(T_1, T_1, T_1), (T_2,T_2,T_2), \dots,  (T_7,T_7,T_7)$. Hence, comparisons can only be done between these 7 sequences. If there was any benefit to receiving different interventions, in a different order, this could not be discovered by PERCS-AB. Notice also that all of the comparisons of PERCS-AB can be done with data collected through PERCS, though this comes at the cost of a reduced sample size. This tradeoff demonstrations again why SRTs are especially well situated for MOOC experimentation.



\subsubsection{Results from PERCS} \label{results_seq}
We now present results answering \ref{rq1}. Since there are a large number of potential sequences, here we focus on the highest-level comparison, i.e., understanding the proper sequence of any email and no email. To do the comparison we look at the proportion of students returning to the course in week 4 (the final week) after receiving a given sequence of emails ($E_1$) and no email ($E_0$), as shown in Figure \ref{fig:seq_results}.

\begin{figure}
\includegraphics[width= \columnwidth]{img/seq.png}
\caption{95\% confidence intervals for the proportion of students returning to the course in week 4 after receiving a given three week sequence of emails ($E_1$) and no email ($E_0$)} \label{fig:seq_results}
\end{figure} 

We note some important observations. For US learners, sequences with emails sent in the first week (e.g.,those sequences which start with $E_1$, the last four columns in Figure \ref{fig:seq_results}), tend to be more beneficial than sequences without. For Indian learners this is not true. 
%and relative to US-based learners Indian learners perform the same or better in conditions where there was not an email sent in the first week (i.e., beginning with $E_0$) and worse in those conditions where there was an email in the first week (i.e., beginning with $E_1$). 
Overall, for both countries, the confidence intervals across sequences are mostly overlapping, indicating that differences in effects of various email sequences are not strongly significant. The size of the confidence intervals change due to the probability of receiving an email ($E_1$) being larger than the probability of not receiving an email ($E_0$).

%Notice also how the size of confidence interval changes based on the number of learners randomized to that group. The sequence of 3 weeks of no emails, $(E_0, E_0, E_0)$ only had a $(\frac{1}{7})^3$ chance of randomization while the sequence of 3 weeks of emails $(E_1, E_1, E_1)$ had a  $(\frac{6}{7})^3$ probability. If this sequence comparison was the primary aim of PERCS, randomization probabilities should change to give more balance across these sequences.

%For PERCS, we were most interested in understanding how to best sequence and space out emails with problems and emails without problems (RQ\ref{rq1}). We were not sure if users would be motivated by only problem-based emails, no-problem email reminders, or no emails at all.  Specifically, we were interested in understanding the sequential differences between the groups: 1) no emails ($E_0$), 2) no problem emails ($P_0$), 3) global problem emails ($P_1$), and 4) cultural problem emails ($P_2$) . Each week, a user could have received one of these four types of emails, providing $4^3$ = 64 sequences to compare (i.e., $(E_0,E_0,E_0), (E_0,E_0,P_0), (E_0,E_0,P_1), \dots (P_2,P_2,P_2)$). For users in each of these sequences, we create a confidence interval for the log number of course clicks throughout the entire course. The results are in table blah

\subsection{Timing}\label{sec:avg-treatment-effects}

\subsubsection{Overview}

Instead of being interested in a sequence of interventions, researchers might want to know about the effect of an intervention option at a particular time point. A treatment that was effective at the beginning of the course may be less effective towards the end of the course. By understanding effects of intervention options at a time point, designers can build adaptive interventions which deliver the optimal treatment at all times. For PERCS, \ref{rq2} from Section~\ref{sec:rqs} regards timing-- which email type is most effective during each week?

%\subsubsection{Research Questions}

%Research questions regarding treatment effects at particular time points include:

%\begin{itemize}
%\item \textbf{Video Optimization}: For the last video in the course, is it better to have the video contain slides only or to also feature the instructor?
%\item \textbf{Content Spacing}: What is the effect of frequent review (compared to no review) during the third set of recommended problems? 
%\item \textbf{PERCS}: Research question \ref{rq2} regards treatment timing.
%\end{itemize}

\subsubsection{Advantages of SRTs}


%For the last video in the course, is it better to have the video contain slides only or to also feature the instructor?
%What is the effect of frequent review (compared to no review) during the third set of recommended problems? 
%How does sending a cultural problem emails in week two effect the subsequent week's course activity, compared to not sending any email?

Answering research questions about treatment timing is done by estimating average treatment effects, i.e., the average effect of a given treatment option at a given time point. Here, the averaging is over all prior treatment received, allowing the effect to be only for the particular time point of interest.

SRTs permit the estimation of average treatment effects at various time points. By re-randomizing individuals, we can separately estimate average treatment effects at each time point and eliminate confounding with treatment delivered previously. In A/B tests, such a comparison is only possible the first time treatment is delivered. At times after the first treatment delivery, because the learner will have received the same treatment at all previous time points, the effect of a given treatment option is confounded with the effects of prior treatment.

To exemplify, in PERCS, to understand which email type is most effective in week 3, we compare the average effect of cultural problem emails in week 3 (any, any, $P_2$) compared to no email in week 3 (any, any, $E_0$). By doing this comparison, we average over all treatments delivered prior to week 3, and isolate the effect of interest to emails only in week 3. In PERCS-AB, such a comparison is impossible. We could only estimate the effects of cultural problem emails for all 3 weeks, to no email for all 3 weeks, ($P_2$, $P_2$, $P_2$) vs ($E_0$, $E_0$, $E_0$). The estimate in PERCS-AB is a compounding effect of cultural problem emails for all 3 weeks vs no email for all 3 weeks, instead of an average effect isolated to week 3.

In SRTs, average treatment effects can also be estimated for outcomes measured \textit{after} the next re-randomization (sometimes called delayed effects).  For example, in addition to understanding the average effect of cultural problem emails in week 2, on week 3 course activity in PERCS, we are also able to understand the average effect of cultural problem emails in week 2, on week 4 course activity (and other outcomes such as course completion). We do so by averaging over both week 1 treatment and week 3 treatment. This delayed effect cannot be estimated in PERCS-AB since, with no re-randomization after week 2, the estimate will be confounded by treatment in week 3.

\subsubsection{Discussion}
%The Difference Between Average Treatment Effects and Sequence Effects

%% I might be able to cut this

Research questions on average treatment effects often seem similar to questions regarding sequence effects. In order to elucidate the differences, below are 3 types of research questions in PERCS:
\begin{enumerate}
    \item What is the effect of a cultural problem email in week three, after not receiving any email prior? Compare ($E_0, E_0, P_2$) vs ($E_0, E_0, E_0$) \label{timing_rq1}
    
    \item What is the average effect of a cultural problem email in week three (averaging over all prior treatment)? Compare (any, any, $P_2$) vs (any, any, $E_0$) \label{timing_rq2}
    
    \item What is the effect of getting a cultural problem email every week until week three? Compare $(P_2, P_2, P_2)$  vs $(E_0, E_0, E_0)$ \label{timing_rq3}
\end{enumerate}

Questions \ref{timing_rq1} and \ref{timing_rq3} are questions of comparing sequences of treatments, while question \ref{timing_rq2} is about average treatment effects. Note that all three questions can be answered by PERCS, but only question \ref{timing_rq3} can be answered by PERCS-AB.

Also, one advantage of analyzing average treatment effects is that the sample size is typically larger than when comparing individual sequences of treatments, since the comparison does not restrict users based on what they received before or after the given week of interest.

\subsubsection{Results from PERCS}

To assess \ref{rq2}, for each week, we perform logistic regression with a binary outcome indicating whether the user clicks anything in the course during the week after receiving an email. The results are in Figure~\ref{avg_eff_results}. Negative values indicate a reduced chance of returning to the course, compared to no email, while positive values indicate an increased chance of returning to the course.

\begin{figure}
\includegraphics[width= \columnwidth]{img/average.png}
\caption{95\% confidence intervals of the log odds ratios of probability of returning to the course in the subsequent week for emails containing no problem, a global problem, or a cultural problem, when compared to being sent no email. {\large*} indicates a moderate effect with significance at $\alpha$ = .2}
\label{avg_eff_results}
\end{figure} 

The results in Figure~\ref{avg_eff_results} show that the impact of emails on Indian learners in weeks 2 and 3 is largely positive, but the impact of receiving a no problem email ($P_0$) is as good or better than receiving either global or cultural problem emails ($P_1$ and $P_2$, respectively). Also, in week 2, emails of all types were moderately effective, indicating this is a good time to send Indian users email reminders for this course.%, but including motivating data science problems in those emails may not be worth the effort.

For US learners, the effects are non-significant across all emails except for the cultural problem email ($P_2$) in the last week of the course, and the log odds ratios are small and in many cases negative. This indicates that for all weeks, emails for US users did not impact their propensity to return to the course, and may even deter them from returning -- a counterintuitive, but important, insight from PERCS regarding timing of communication with learners.

\subsection{Personalizing}\label{sec:personalization-with-srts}

\subsubsection{Overview}
%\TN{This should match beginning}
SDLEs are notable for the high degree of diversity both across and within learners \cite{Kizilcec_2013,Kizilcec_2017}. Due to this diversity, we might expect intervention effectiveness to vary along with relevant learner attributes. If an intervention works for a specific user at a given time, that intervention may not be effective for a different user, or even the same user at a different time.  Personalizing treatment, by discovering when and for whom certain treatments are most effective, is critical. For PERCS, \ref{rq3} from Section~\ref{sec:rqs} regards personalization-- are certain emails more effective for active learners?

In clinical trials, learning how to personalize treatment is synonymous with discovering \emph{moderators} \cite{Kraemer_2002}. Moderators are subject-specific variables which change the efficacy of an intervention. For example, if a MOOC intervention works better for older users than younger users, then age is a moderator and can then be used to personalize the intervention; one may deliver the intervention to older learners. Answering \ref{rq3} in PERCS is equivalent to understanding if previous course activity is a moderator of email effectiveness.
%
%\subsubsection{Research Questions}
%
%Research questions about moderator discovery for treatment personalization include:
%
%\begin{itemize}
%\item \textbf{Video Optimization}: If a learner watched a slide only video and then performed poorly, should they now be shown videos featuring the instructor?
%\item \textbf{Content Spacing}:  Do learners who are performing well throughout the course need to receive different review problem spacing sequences than poor performing learners? 
%\item \textbf{PERCS}: Research question \ref{rq3} regards treatment personalization.
%\end{itemize}
\subsubsection{Advantages of SRTs}

Some moderators can be discovered using A/B trials, however, SRTs permit the discovery of two other types of moderators: baseline moderators for additional sequences and mid-course moderators.

%Add jjw cite on personalization with RL - talk about how it can discover things to personalize on, not prespecify
\textbf{Baseline sequence moderators.} Baseline variables are measured prior to the first treatment randomization. Baseline variables include learner demographics (e.g., gender, location, age) and course activity measured prior to the first randomization (e.g., whether the users has taken the course previously, scores on early assignments, survey responses at the beginning of the course). Often these variables moderate the effect of treatments and can be used for personalization. Discovering baseline moderators helps understand how to personalize interventions to account for diversity across learners.

SRTs and A/B tests both permit the discovery of baseline moderators. However, in SRTs, because users receive a larger variety of intervention sequences (see Section \ref{sec:optimal-sequence}), this permits the discovery of baseline moderators for effects of each of these sequences. This leads to a richer and more specific understanding of the moderating effects of various learner characteristics.  For example, unlike PERCS-AB, we can evaluate how a learner's location moderates the effect of each email sequence analyzed in Section~\ref{results_seq}

%As an example, in both PERCS and PERCS-AB, one could answer the question: is the effect of 3 weeks of cultural problem emails different for Indian learners compared to US learners? However, in PERCS, one is able to evaluate the moderation of learners' location on a larger variety of treatment sequence comparisons. Indeed, the PERCS design allows an experimenter to evaluate the moderation of location on every possible sequence of interventions in the trial.  One could also answer questions about how location moderates treatment sequence efficacy: is the effect of sequences which vary cultural and global problem emails different for Indian learners compared to US learners? PERCS-AB is not able to answer this second question since no users are re-randomized to receive both cultural and global emails throughout the course. PERCS-AB is only able to evaluate moderation of baseline variables on the small number of sequences in the trial.

%% Could put in examples from other example trials here if it warrants more explanation
\textbf{Mid-course Moderators.} Baseline moderators are important for personalizing initial treatment (or treatment sequences), however, understanding how to change treatment based on variables measured throughout the course -- mid-course moderators -- is critical. Discovering mid-course moderators tells practitioners how to personalize interventions throughout the course to account for heterogeneity both across different users and within a user over time. 

Unlike A/B tests, SRTs permit the discovery of mid-course moderators. Statistically, due to bias introduced when including post-randomization variables in analyses, one can only discover moderator variables measured prior to randomization \cite{Kraemer_2002}. If all learners were only randomized once, potential moderators measured after the first treatment cannot be discovered. By re-randomizing in SRTs, moderators measured before each of the randomizations (which now includes mid-course data) can be discovered. 

%<Should I further explain here the specifics, like I still have to preserve ordering, I can only assess there moderation on future treatment>

%Are certain data science problem emails more or less effective for active learners?

%we hypothesized that growth mindset framing in emails sent at the end of week three only works well for students who were inactive during week 3, because they would benefit from the growth mindset encouragement. Because users were randomized again at the end of week 3, we can use PERCS data to assess how week 3 activity moderates the effect of growth mindset emails (sent at the end week 3) on week 4 activity. In PERCS-AB, week three course activity cannot be assessed as a moderator in PERCS-AB since it was measured after the one and only randomization in week one. 

Because users were randomized again at the end of week three, to answer \ref{rq3} about emails sent during week three, we can use PERCS data to assess how activity during week three moderates the effect of data science problem emails (sent at the end week three) on week four activity. In PERCS-AB, week three course activity cannot be assessed as a moderator since it is measured after the one and only randomization in week one. 

\subsubsection{Discussion}

We can also evaluate mid-course moderators that include previous treatment. For example, we may think that responsiveness to previous treatment could inform how to personalize future treatment. Those that were responsive should continue getting the same treatment while those that were non-responsive should get assigned different treatment. In PERCS, for example, we might expect week two emails to benefit users who responded positively to emails in week one. One could assess this by comparing two groups: Group 1 are users who received an email ($E_1$) but did not click in the course afterwards (i.e., email non-responders). Group 2 are users who received an email ($E_1$) but did click in the course afterwards (i.e., email responders). We could compare the effect of emails in week two for Group 1 vs Group 2.


%In PERCS, we hypothesized that growth mindset emails are more effective for users indicating they liked growth mindset in the previous week and users indicating they did not like non-growth mindset in the previous week. More specifically, there are four groups of learners: Group 1 are learners who received growth mindset framing in week one and had course activity in week two (i.e., growth mindset responders), Group 2 are learners who received growth mindset framing in week one and had no course activity in week two (i.e., growth mindset non-responders), Group 3 are learners who received no growth mindset framing in week one and had course activity in week two (i.e., no growth mindset responders), Group 4 are learners who received no growth mindset framing in week one and had no course activity in week two (i.e., no growth mindset non-responders). We expected growth mindset framing in week two emails to benefit Groups 1 and 4 more than Groups 2 and 3. By re-randomizing at the end of week two, we assess moderation by comparing treatment effects of growth mindset framing in week two emails for Groups 1 and 4 vs Groups 2 and 3.

Discovering how to personalize based on mid-course activity is one of the major benefits of SRTs. These discoveries allow educators to select interventions that meet the needs of learners as they transition throughout the course. Also, as learning content optimization starts to happen in real-time (i.e., reinforcement learning), knowing which real-time variables to measure and use for online optimization is critical. SRTs permit this discovery.

%\TN{sentence like this here but for within leaners: Discovering baseline moderators helps understand how to personalize interventions to account for heterogeneity between different learners.}

\subsubsection{Results from PERCS}

\begin{figure}
\includegraphics[width = \columnwidth]{img/moderator_plot.png}
\caption{95\% confidence intervals of the log odds ratios of probability of returning to the course in the subsequent week for emails containing no problem, a global problem, or a cultural problem, when compared to being sent no email, The log odds ratio is calculated for users who had activity (active) or did not have activity (inactive) in the prior week.} \label{fig:moderator}
\end{figure}

For PERCS, we were most interested in previous week's course activity as a mid-course moderator. We wanted to see how different types of emails effect active and inactive users differently. Active users are defined as users who had one or more clicks in the course during the previous week. Before the trial, we did not know if problem-based emails would encourage inactive users (because they need the motivational reminder) or discourage inactive users (because the problem may be too advanced). To assess this, in Figure~\ref{fig:moderator} we plot the log odds ratios of the probability of returning to the course in the subsequent week for different emails conditions, compared to the control of no email. A positive log odds ratio indicates users had a higher chance of returning to the course after receiving the corresponding email problem type (compared to the no email control).

%There are two key observations drawn from the results in 
In week one, for both US and Indian learners, reminder emails of all types performed better for active users than inactive users (higher log odds for blue than magenta, Figure~\ref{fig:moderator}). In week three, the sign of the moderation switched, as emails performed better for inactive users compared to active users (higher log odds for magenta than blue). The difference was larger for Indian learners. Also, the log odds ratios for inactive users were positive, while the log odds ratios for active users were negative. To ensure we encourage inactive users to return to the course while not discouraging active users, email sending should adapt based on both users' previous course activity and the course week.

\section{Implications for Practice}\label{sec:implications-for-practice}

This section outlines some useful considerations for researchers who are interested in designing and running SRTs for SDLEs. First, before thinking about trial specifics, researchers should always remember that experiments are created to inform scientific understanding and answer questions about interventions. Deciding if a SRT is the correct trial design depends purely upon the scientific questions of interest. For example, if researchers are not interested in understanding how to sequence, time, and personalize interventions, running a SRT is unnecessary. In PERCS, if a researcher were interested in only comparing two sequences of interventions then it may be best to run an A/B test on those two sequences and forgo answers to other questions. 

In situations where a SRT is appropriate, there are also important trial design considerations.  All intervention sequences in a SRT should be useful, feasible, and scalable. It is useless to evaluate intervention sequences which could never be done in practice or which are knowingly deleterious to subjects. For example, suppose a researcher was curious about optimal ordering of course content and, in turn, sequentially randomized learners to various sequences of content. If content B requires information taught in content A, none of the sequences in the experiment should place content B before content A. As another example, in PERCS, because the MOOC platform does not currently support fully-automated, scheduled delivery of email, messages were only sent once per week. We did not explore the possibility of sending emails many times per week (e.g., re-randomizing email sending every day) because, in practice, interventions which require manual daily email sending would not currently be feasible for instructors on this platform.

As in any other trial design, sample size and power calculations are important for SRTs. Sample size calculations should be based off of the most important research questions the trial intends to answer. Since there are a larger number of possible treatment sequences in a SRT, calculating power and sample size requires researchers to consider which subset of users will be randomized to the sequences of interest. Then, sample size calculations are similar to A/B tests for both comparing interventions and discovering moderators \cite{Oetting_2011}. 
Due to the larger space of potential treatment sequences, sample sizes usually need to be larger for SRTs (compared to A/B tests). To increase power, researchers may consider changing randomization probabilities to favor interventions of interest. 
%For example, in PERCS, if our primary interest was in comparing cultural problem emails to global problem emails, we might change the weekly randomization probabilities in Table \ref{tab:probs} to favor these two interventions.



\section{Discussion}

Adapting, sequencing, and personalizing interventions is critical to meet the diverse needs of learners in SDLEs. When designing adaptive interventions, experimentation is useful for evaluating and comparing possible sequences. Unfortunately, single-randomized A/B tests cannot answer questions about ways to adapt and sequence interventions throughout a course.  In this work, we demonstrated how a new type of experimental design, SRTs, are valuable for developing adaptive personalized interventions in SDLEs. SRTs provide answers to questions regarding treatment sequencing, timing, and personalization throughout a course. Answers to these questions will both improve outcomes for learners and deepen understanding of learning science in scalable environments.

In this work, we provided a few examples of different SRTs. There are many more variations of SRTs that are useful for answering additional research questions. In PERCS, all users have the same randomization for all three weeks. However, if a certain learner is evidently responding well to treatment, it may not make sense to re-randomize them and change their current treatment. Many Sequential Multiple Assignment Randomized Trials (SMARTs) \cite{Murphy_2005, Pelham_2016} solve this issue by varying second stage randomizations based on a subject's response to prior treatment. This design is useful when moderators are known beforehand. It's important to note that these changes in randomization are pre-specified and intended for exploring adaptive interventions, not online optimization.

Other variations of SRTs may be useful to answer research questions in SDLEs. Since many online courses are accessible to learners at any time, randomization timing could be based on when each user enters the course (randomized one, two, and three weeks from the day the user enrolls in a course). If treatment delivery timing is a research question, the delivery time can also be (re)randomized (i.e., each week of the course, re-randomize users to receive one weekly email or seven daily email reminders). Also, since many SDLEs provide learners with all course content at the beginning of the course, a trial aiming to re-randomize course content could use trigger-based re-randomizations--where users' future content is only changed after they have watched a certain video or completed a particular assignment--to prevent early exposure to future treatment.

%In addition to content access, SDLEs have other unique aspects. In online courses, users can often enter an online course at any time.  In an A/B test, if randomization to treatment occurs during the course start date, users enrolled after that date will not be used in the study. In SRTs, since users will be randomized again at later times, the late enrolling students could potentially be used in these later randomizations. However, thoughtful analysis and statistical methodology needs to be developed to ensure proper estimation of treatment effects.

Though useful, SRTs have limitations. SRTs are non-adaptive trial designs. If an experimenter wishes to both learn efficacious treatments and provide benefit to learners in the current trial, adaptive designs such as \cite{Williams_2018} would be more appropriate. Combining adaptive designs with SRTs may also be useful for both developing high-quality adaptive interventions and improving benefits for current learners \cite{Cheung_2015}.

PERCS also had some limitations. For one, during our first iteration of the trial, the emails contained syntax errors, and some treatment groups did not receive emails. These errors were fixed for future iterations and the error-free iterations were the ones used in our analysis. Secondly, since some users (10\%) retook the online course multiple times, those users were repeated in multiple iterations of the trial. Lastly, it's important to note that PERCS was an exploratory trial not a confirmatory trial. The goal of PERCS was to explore several sequences of treatments and evaluate their efficacy for different learners. The next step for PERCS is to narrow down best treatment options based on current data (which may be different for Indian and US learners). Since the current evidence is not extremely strong, we would then run a second SRT with fewer treatments, acquiring more data on those treatments of interest. Once we have enough evidence to suggest which sequence of emails is optimal, we can then compare this learned optimal sequence of emails to a control in an A/B test confirmatory trial. Treatment A would be the hypothesized optimal adaptive sequence of emails and treatment B would be no email.



%\pagebreak
%\pagebreak

%\subsection{nonsense}

%

